DAG-width is PSPACE-complete

Berwanger et al. show that for every graph $G$ of size $n$ and DAG-width $k$ there is a DAG decomposition of width $k$ and size $n^{O(k)}$. This gives a polynomial time algorithm for determining the DAG-width of a graph for any fixed $k$. However, if the DAG-width of the graphs from a class is not bounded, such algorithms become exponential. This raises the question whether we can always find a DAG decomposition of size polynomial in $n$ as it is the case for tree width and all generalisations of tree width similar to DAG-width. We show that there is an infinite class of graphs such that every DAG decomposition of optimal width has size super-polynomial in $n$ and, moreover, there is no polynomial size DAG decomposition which would approximate an optimal decomposition up to an additive constant. In the second part we use our construction to prove that deciding whether the DAG-width of a given graph is at most a given constant is PSPACE-complete.

==> abbrs.tex <==
% Abbreviations for \calX, \frakX, \bbX etc. in math mode.
\makeatletter
\newcommand{\@abbrev}[3]{
  \def\c@a@def##1{
      \if ##1.
        \relax
      \else
        \@ifdefinable{\@nameuse{#1##1}}{\@namedef{#1##1}{#2##1}}
        \expandafter\c@a@def
      \fi
    }
  \c@a@def #3.
}
\@abbrev{bb}{\mathbb}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}
\@abbrev{bf}{\mathbf}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\@abbrev{bit}{\boldsymbol}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\@abbrev{cal}{\mathcal}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}
\@abbrev{frak}{\mathfrak}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\@abbrev{rm}{\mathrm}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\@abbrev{scr}{\mathscr}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}
\@abbrev{sf}{\mathsf}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\@abbrev{Alg}{\Alg}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}
\@abbrev{Str}{\Str}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}
\@abbrev{set}{\mathbb}{ABCDEFGHIJKLMNOPQRSTUVWXYZ}
\@abbrev{tup}{\tup}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\@abbrev{tld}{\tilde}{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}
\makeatother

\newcommand{\red}[1]{\textcolor{red}{#1}}

==> app-bigDAG.tex <==
\section{The Complexity of DAG-width and DAG-width Game}

\subsection{Outline of this section}
For didactical reasons we prove our results about the complexity of DAG-width 
and DAG-width games in a different order than in the paper. First we show that 
there are graphs $G$ whose all DAG decompositions of optimal width are 
super-polynomial in $|V(G)|$. Then we generalise this construction to prove 
that allowing the width of a decomposition be sub-optimal (with an error up to 
an additive constant) does not help to consruct polynomial decompositions.

Next we use our construction to prove that $\DAGWprob$ is \conp-hard, which is 
one part of our proof of \pspace-hardness, namely the simulation of the moves 
of the universal player by universal levels. Finally, we extend the 
construction by introducing existential levels where the choice of the 
existential player is simulated.

\subsection{Big DAG Decompositions}

Let $s,t\colon \bbN \to \bbN$ be two monotonically non-increasing
functions with $2\le s(n) < n/\log n$ and $2\le t(n)$ for
all~$n\ge5$. We define a class of graphs $G_n(s,t)$ of \dagw~$n+1$
such that every DAG decomposition of width $n+1$ has
super-polynomially many bags in the size of $G_n(s,t)$ (measured in
the number of vertices), which is in $O(n^2\cdot t(n)) = O(n^2\cdot t(n))$. The
parameter~$s$ will be used to determine the difference between the
optimal width of a DAG decomposition and the best possible width of a
polynomial size decomposition. The parameter~$t\ge 2$ is used for
fine-tuning. Our proof works already if $s(n) = t(n) = 2$ for all~$n$
and the reader is invited to assume these values at first. We shall
consider what changes if~$s$ and~$t$ are different later.

For $n\in\{1,\ldots,4\}$, $G_n(s,t)$ the graph $G_1(s,t)$ is a single
vertex without edges. For $n\ge 5$, the graph $G_n(s,t)$ is
constructed as follows (see Figure~\ref{fig:graph}).  Let $M(n)$ and $C_i(n)$ 
for
$i\in\{0,\ldots,t(n)-1\}$ be pairwise disjoint sets of vertices, each of
$n-s(n)$ elements. Let $D^s(n)$ be a set of~$s(n)$ elements disjoint from
all $C_i(n)$ and $M(n)$, and let $N(n) = M(n) \cup D^s(n)$. Let $A^s(n)$ be a 
set
of~$s(n)$ new vertices, and let $B^t(n) = \{b_0(n),\ldots,b_{t(n)-1}(n)\}$ be a
set of~$t(n)$ new vertices.  The graph $G_n(s,t)$ has vertices
\[V(G_n(s,t)) = V(G_{n-s(n)-1}(s,t)) \cupdot A^s(n) \cupdot B^t(n) \cupdot
\bigcup_{i = 0}^{t(n)-1} C_i(n)\cupdot N(n)\,.\]
 We say that vertices from $A^s(n) \cup B^t(n) \cup \bigcup_{i = 0}^{t(n)-1} 
C_i(n) \cup N(n)$
are in level~$n$. The edges are defined by
\begin{align*}
E(G_n(s,t)) = &E(G_{n-s(n)-1}(s,t)) \cup {N(n) \choose 2} \cup 
\bigcup_{i=0}^{t(n)-1}
{C_i(n) \choose 2} \cup {A^s(n) \choose 2}\\
                     &\cup \bigcup_{i=0}^{t(n)-1} \Bigl( \bigl(N(n) \times
                     C_i(n)\bigr) \cup \bigl(C_i(n) \times D^s(n)
                     \bigr) \cup \bigl(C_i(n) \times
                     \{b_i(n)\}\bigr) \Bigr)\\
                    & \cup
                     \bigl(B^t(n) \times A^s(n)\bigr) \cup
                     \bigl(A^s(n) \times B^t(n) \bigr)\cup \bigl(A^s(n) \times 
M(n)\bigr)\\
                    & \cup \bigl(N(n) \times V(G_{n-s(n)-1}(s,t))\bigr) \cup 
\bigl(A^s(n)
                     \times V(G_{n-s(n)-1}(s,t))\bigr)\\
                    & \cup \bigl( V(G_{n-s(n)-1}(s,t))
                     \times A^s(n) \bigr) \cup \bigl(V(G_{n-s(n)-1}(s,t)) \times 
B^t(n)\bigr)\,.
\end{align*}
In other words, the first line says that $G_n(s,t)$ has all edges from
$G_{n-s(n)-1}(s,t)$, and that $N(n)$, all~$C_i(n)$
for $i\in\{0,\ldots,t(n)-1\}$ and $A^s(n)$ are cliques of sizes~$n$, $n-s(n)$
and~$s$, respectively. Note also that $B^t(n)$ induces an independent set.


\begin{figure}
  \centering
  \begin{tikzpicture}
    \node[draw,circle,inner sep=5mm] (C_0) at (0,0){$M$};
    \node[gray] at (0,-0.4){$n-s(n)$};

    % \node[vertex] at (2,0){};
    %   \node at (2.5,0){$\cdots$};
    % \node[vertex] at (3,0){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (D) at 
(2.5,0){$D^s$};
       % \node at (3,0.5){$D^s$};
  \draw (C_0) -- (D);

    \node[draw,circle,inner sep=5mm] (C_1) at (3,-3){$C_0$};
    \node[gray] at (3,-3.4){$n-s(n)$};
      \node at (5,-3){$\cdots$};
    \node[draw,circle,inner sep=2.6mm] (C_t) at (7,-3){$C_{t(n)-1}$};
    \node[gray] at (7,-3.4){$n-s(n)$};
   \draw[-slim] (C_0) to (C_1);
   \draw[-slim] (C_0) to (C_t);
   \draw[-slim] (D) to (C_1);
   \draw[-slim] (D) to (C_t);
   \draw[-slim,bend right] (C_1) to (D);
   \draw[-slim,bend right] (C_t) to (D);

    % \node[vertex] at (-3.5,-2){};
    %   \node at (-3,-2){$\cdots$};
    % \node[vertex] at (-2.5,-2){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (A) at 
(-3,-2){$A^s$};
       % \node at (-4,-1.5){$A^s = \{a^1,\ldots,a^s\}$};
    \draw[-slim] (A) to (C_0);

  \node[vertex] (b_1) at (-4,-5){};
    \node at (-3,-5){$\cdots$};
  \node[vertex] (b_t) at (-2,-5){};
    \node[draw,ellipse,minimum height=5mm,minimum width=30mm] (B) at
    (-3,-5){};
  \node at (-5.2,-5.5){$B^t = \{b_0,\ldots,b_{t(n)-1}\}$};
  \draw (B) to (A);
  \draw[-slim,bend left=40] (C_1) to (b_1);
  \draw[-slim,bend left=40] (C_t) to (b_t);

   \node[draw,rectangle,minimum width=20mm,minimum height=15mm]
   (G_n-3) at (0,-3){$G_{n-s(n)-1}(s,t)$};
   \draw[-slim] (C_0) to (G_n-3);
   \draw[-slim] (D) to (G_n-3);
   \draw            (A) to (G_n-3);
   \draw[-slim] (G_n-3) to (B);



  \end{tikzpicture}
  \caption{The construction of $G_n(s,t)$. Indices $\cdot(n)$ are omitted.}
  \label{fig:graph}
\end{figure}

For the following lemma the precise definition of~$s$ and $t$ in
$G_{n-s(n)-1}(s,t)$ is inessential.

\begin{lemma}
  \label{lemma:dagw}
The \dagw of $G_n(s,t)$ is $n+1$.
\end{lemma}
\begin{proof}
  The cops have the following winning strategy for the \dagw game on
  $G_n(s,t)$. First they occupy $N(n)$ and we can assume that the
  robber chooses some $C_i(n)$ (for $i\in\{0,\ldots,t(n)-1\}$) because all
  other strongly connected components of $G_n(s,t) - N(n)$ have
  incoming edges from all~$C_i(n)$. (So the robber can go
  to every other vertex that is reachable now also later, see Lemma~5.21
  in~\cite{RabinovichPhD}.)  Then the remaining cop occupies $b_i(n)$. If
  the robber stays in $C_i(n)$, the cops from $M(n)$ capture him there
  (recall that $M(n)$ has the same size $n-s(n)$ as every $C_i(n)$,
  $i\in\{0,\ldots,t(n)-1\}$). So we can assume that the robber goes to
  $A^s(n) \cup (B^t(n)\setminus\{b_i(n)\})$ (again, there is no reason for him 
to go directly to
  $G_{n-s(n)-1}(s,t)$). If the robber remains in $B^t(n)$, he is captured in 
the next move. The cops from $D^s(n)$ move to $A^s(n)$ and
  force the robber to proceed to $G_{n-s(n)-1}(s,t)$. From now on, the $s+1$
  cops in $A^s(n) \cup \{b_i(n)\}$ stay there until the end of the play
  and the remaining $n-s(n)$ cops play in $G_{n-s(n)-1}(s,t)$ in the same
  way as on $G_n(s,t)$ until the robber is captured or expelled to a
  $b_j(n)$ for $j\neq i$. There he will be captured in one move. Note
  that $G_{n-s(n)-1}(s,t)$ has outgoing edges only to $B^t(n)$ and to $A^s(n)$.

  A winning robber strategy against~$n$ cops is to stay in $N(n)$
  until all~$n$ cops are there and then to go to $C_0(n)$. In that
  position of the game, no cop can be removed from his vertex due to
  the monotonicity winning condition.
\end{proof}

We now prove that the described winning strategy for~$n+1$ cops (let
us call it~$\sigma$) is the only possible one up to some irrelevant
changes. Then we count the number of positions that are consistent
with~$\sigma$ and observe that there are super-polynomially many of
them. It will follow that every DAG decomposition of the optimal width
has a super-polynomial size.

The first kind of change is to occupy the sets $M(n)$, $C_i(n)$
($i\in\{0,\ldots,t(n)-1\}$), $A^s(n)$ and $D^s(n)$ in a different order
than according to~$\sigma$,
which, obviously, makes no sense, as~$\sigma$ prescribes to occupy
either the whole set or none of its vertices and those vertices have
ingoing and outgoing edges from and to the same vertices. The second
kind of a change is to place cops on and then to remove them from
vertices that are already unavailable for the robber. (Note
that~$\sigma$ never lets cops stay on such vertices.) This is also
useless because of the monotonicity. Both changes can obviously only
increase the number of possible positions.

\begin{lemma}\label{lemma:decs_and_positions}
If there is a DAG decomposition of a graph $G$ of width $k$ and of
size $n$, then $k$ cops have a winning strategy such that the number
of positions consistent with this strategy is at most~$n\cdot |G|$.
\end{lemma}
\begin{proof}
  Consider the strategy (let us call it $\sigma$) obtained from a DAG
  decomposition of width $k$ as described in \cite[Theorem
  16]{BerwangerDawHunKreObd12}. In a play consistent with~$\sigma$, the
  cops occupy only sets of vertices that correspond to some bag. Thus
  there are at most $n$ cop placements that can appear in a play. A
  position can be described by the cop placement and the robber
  vertex. There are at most $|G|$ vertices, so the total number of
  positions is at most $n\cdot |G|$.
\end{proof}


\begin{theorem}\label{thm:super-poly}
Every DAG decomposition of $G_n(s,t)$ of width $n+1$ has
super-po\-ly\-no\-mial\-ly many bags.
\end{theorem}
\begin{proof}
We describe the strategy of the robber that enforces the cops to play
according to~$\sigma$ up to irrelevant changes. If $n+1$ cops play in
a different way, they lose.

The robber remains in $N(n)$ until it is completely occupied by cops. If
a cop was placed on a vertex $v\notin N(n)$ before $N(n)$ was
completely occupied, the cops lose. Indeed, consider the position
where all vertices of $N(n)$ are occupied for the first
time. Because~$v$ (whatever it is) has been occupied and because it is
still reachable now from $N(n)$, the last $(n+1)$-st cop is still
on~$v$, otherwise the monotonicity is violated. The robber goes to
some $C_i(n)$ from which~$v$ is reachable via paths avoiding $N(n)$
(such a $C_i(n)$ always exists) and the cops have no legal move. Thus
the first moves of the cops are to occupy $N(n)$ and the last cop
remains outside of the graph.

The robber chooses some $C_i(n)$ and the cops have no other possible
move than to place the last remaining cop on $b_i(n)$ (otherwise we have the
situation discussed in the previous paragraph). The robber goes to
$A^s(n)\cup B^t(n)\setminus \{b_i(n)\}$. In this position, the cops in 
$\{b_i(n)\} \cup M(n)$ cannot
be removed and all $C_i(n)$ are unavailable for the cops. So the cops
from $D^s(n)$ must be used and they can be placed either in $A^s(n)$
or in $G_{n-s(n)-1}(s,t)$, or in $B^t(n)\setminus \{b_i(n)\}$. If at least one 
cop is placed in $G_{n-s(n)-1}(s,t)$ or in $B^t(n)\setminus \{b_i(n)\}$, the 
robber remains in $A^s(n)$ until all cops are
placed. Then the cops have no legal move and lose. It follows that the
cops must occupy the whole $A^s(n)$ and the robber goes to
$G_{n-s(n)-1}(s,t)$. From now on, all cops occupying $A^s(n)$ and
$b_i(n)$ will be reachable from the robber vertex and must stay
there. It follows by induction on~$n$ that~$\sigma$ is the unique
winning strategy for $n+1$ cops up to irrelevant changes.

We now count the number of positions that are consistent
with~$\sigma$. When the robber goes to the last level, the cops are
occupying $A^s(\ell)$ for all levels $\ell$ that appear as
indices of $G_\ell( s,t)$. Additionally, for each $\ell$, the cops
occupy exactly one of $\{b_0(\ell),\ldots,b_{t(\ell)}(\ell)\}$. (If they
occupy more of them, the remaining cops do not suffice to capture the
robber due to \Cref{lemma:dagw}.)  Thus when the robber is in the
lowest level of the recursion, there are $t^{\#\ell}$ positions where
$\#\ell$ is the total number of levels in the graph and $t = \min
\{t(\ell) \mid~\ell \text{ is a level in }G_n(s,t)\}$. As
$s(\ell)<\ell/\log \ell \le n\log n$, there are at least $\log n$
levels, \ie $\#\ell \ge \log n$ and the number of bags is at least
$t^{\log n}$. 

The size of $G_n(s,t)$ is 
\begin{align*}
|G_n(s,t)|& = |N(n)| + t(n)\cdot |C_i(n)| + |A^s(n)| +
|B^t(n)| + |G_{n-s(n)-1}(s,t)|  \\
&= n + t(n)\cdot (n-s(n)) + s(n) + t(n) + |G_{n-s(n)-1}(s,t)|
= O(n^2\cdot t(n))\,,
\end{align*}
 so $t^{\log n}$ is super-polynomial in
$|G_n(s,t)|$ for $\log n\le t\le n$.

Consider a DAG decomposition $\calD$ of $G_n(s,t)$ of width
$n+1$. Towards a contradiction assume that~$\calD$ has at most
$|G_n(s,t)|^c$ bags where~$c$ is a constant. Then the winning strategy
for $n+1$ cops induced by~$\calD$ has at most $|G_n(s,t)|^{c+1}$
positions. We have seen, however, that the number of positions consistent
with~$\sigma$ is super-polynomial in $G_n(s,t)$. 
\end{proof}

\subsection{Consider an Additive Constant Error}

In the simplest case we can set $s(\ell)= t(\ell) = 2$ for all
levels. Then we obtain at least $\lfloor n/2 \rfloor$ levels and the
size of an optimal decomposition is at least
$2^{O(\sqrt{|G_n(s,t)|})}$.  However, at the cost of one additional
cop we can construct a DAG decomposition with polynomially many
bags. We change~$\sigma$ to occupy $A^s(n)$ with two cops instead of
placing one cop on $b_i(n)$. We need one extra cop for this, but this
is not repeated in each level. Already in the first level, when the
robber goes to $G_{n-s(n)-1}(s,t) = G_{n-3}(s,t)$, we have cops only
on $A^s(n)$, but not
on~$b_i(n)$. So one cop is saved for $G_{n-3}(s,t)$ and we can
continue to play in all levels in the same manner.

We can change our choice of~$s$ and $t$ to make the number of
additional cops needed to obtain a polynomial size decomposition
unbounded. Let $s(\ell) = t(\ell) = \lfloor \ell/\log \ell\rfloor$ for
all~$\ell$. Then there are at least $\log n$ levels and
\begin{align*}
  |G_n(s,t)| = &\sum_{i=0}^{t(n)-1}(|C_i(n)| + |\{b_i(n)\}|) + N(n) +
                                                     |A^s(n)|  + 
|G_{n-s(n)}(s,t)|\\
                      & = (n -s(n) + 1)\cdot t(n) + n + s(n) +
                                                     |G_{n-s(n)-1}(s,t)|\\
                      & = O\left(\frac{n^2}{\log n}\right) + |G_{n-s(n)-1}(s,t)|
                                  = O(n^2)\,.
\end{align*}
It remains to estimate the number of bags in an optimal
decomposition. Let $n_1,n_2,\ldots$ be the indices in $G_{n_i}(s,t)$
appearing in $G_n(s,t)$, \ie $n_0 = n$, and for $i>0$ we have $n_i =
n_{i-1} - \lfloor n_{i-1}/\log n_{i-1} -1\rfloor$. Then for $n\ge 5$, \[n_i \ge 
n -
i\cdot n/\log n - i\,,\] which is easy to prove by induction
on~$i$. For all $i\le \log n/2$ we have 
\[n_i \ge n - \frac{\log n}{2}\cdot \frac{n}{\log n} -\frac{\log n}{2}
= \frac{n-\log n}{2} \] 
and thus for $n\ge 5$,
 \[t(n_i) =
\left\lfloor\frac{n_i}{\log n_i}\right\rfloor \ge \frac{(n-\log n)}{2\log n} \ge
\frac{n-n/2}{2\log n} \ge \frac{n}{4\log n}\,.\] So for $\lfloor\log
n/2\rfloor$ many levels $t(n_i) \ge n/(4\log n)$ and thus the number
of bags in any DAG decomposition is at least $(\frac{n}{4\log
  n})^{\lfloor\log n/2\rfloor}$.


We can define a winning cop strategy with only
polynomially many positions with the same trick as before investing
$s(n)-1$ new cops, \ie using $n+s(n)$ cops. Occupy $N(n)$ and when the
robber goes to some $C_i(n)$, occupy $A^s(n)$. The robber has to go to
the lower levels (otherwise he will be captured in
$C_i(n)\cup\{b_i(n)\}$ or in $B^t(n)$) and we do not need cops in
$B^t(n)$. In the following theorem we show that less than $n+s(n)$ cops
do not have a winning strategy with polynomially many positions. Thus
there is no polynomial approximation of an optimal DAG decomposition
by an additive constant.

\begin{theorem}
  For all $G_n(s,t)$ with $n\ge 25$, every DAG decomposition of width at most 
$n-s(n)-1$
  has size at least $\left(\frac{\log n}{16}\right)^{\log n/4}$.
\end{theorem}
\begin{proof}
  We describe a robber strategy against $n-s(n)-1$ cops that allows
  him to enforce at least $(\frac{n}{4\log n})^{\lfloor\log
    n/2\rfloor}$ positions (dependent on his choices of
  $C_i(\ell)$). The robber waits in $N(n)$ until it is occupied
  by~$n$ cops and goes to some $C_i(n)$ for $i\ge 0$ such that $b_i(n)$
  is not occupied by the cops. As $|C_i(n)| = n-s(n) \ge s(n)$ (recall that
  $n\ge 25$) and only $s(n)-1$ cops are left, in all
  $C_i(n)$ there is a cop free vertex. Similarly, the remaining~$s(n)-1$
  cops cannot occupy all $b_i(n)$ (there are $t(n) = s(n)$ many of them), so 
going to such a $C_i(n)$ is
  possible. Now the cops in $N(n)$ cannot move, $s(n)-1$ free cops
  cannot expel the robber from $C_i(n)$ and the robber waits in
  $C_i(n)$ for $b_i(n)$ to be occupied. When the cops announce to do
  this, he runs via $b_i(n)$ and $A^s(n)$ (which also has a free
  vertex) to $G_{n-s(n)-1}(s,t)$ and plays there in the same
  way recursively.

  If the cops do not occupy all vertices in $A^s(n)$ when the robber
  is in the subgraph $G_{n-s(n)-1}(s,t)$, they cannot use the cops
  from $M(n)$, so they cannot expel the robber from $M(n-s(n)-1)$
  (\ie $M$ in the highest but one level). Indeed, $|M(n-s(n)-1)| =
  (n-s(n)-1) - \left\lfloor \frac{n}{\log(n-s(n)-1)} \right\rfloor$
  and there are at most $(n+s(n)-1) - (n-s(n)) - 1 = 2s(n)-2$ free
  cops (namely $n-s(n)$ cops are in $M(n)$ and~$1$ cop is on
  $b_i(n)$), so we only need to choose an appropriately large~$n$, the
  least possible being~$25$. Hence we can assume that the
  cops occupy all $A^s(n)$, \ie $s(n)+1$ cops are tied in level~$n$ and
  there are at most $(n+s(n)-1) - s(n) - 1 = n-2$ cops for
  $G_{n-s(n)-1}(s,t)$.

  Let us count the number of possible positions that may appear in a
  play consistent with the described strategy of the robber. We first
  count the number of levels~$\ell$ where the cops have more than one
  cop in $B^t(\ell)$. When playing according to~$\sigma$, which uses
  $n+1$ cops, exactly one cop is in each $B^t(\ell)$ and now we have
  $s(n)+2$ cops more, so there are at least $\log n/2$ levels $i$ with
  $t(n_i)\ge n/(4\log n)$. Then there are $\log n/4$ levels $\ell$ with at
  most $4n\log^2 n$ cops in each of them. In order to cover
  $B^t(\ell)$ in each such level with $4n\log^2 n$ cops, we need
  $\frac{t(\ell)}{4n/\log^2 n}$ times. As $t(\ell)\ge n/(4\log n)$, we
  obtain $\frac{t(\ell)}{4n/\log^2 n} \ge \frac{\log n}{16}$. Summing
  up, there are $\log n / 4$ levels where the cops have to choose one
  among at least $\log n/16$ placements depending of the robber's
  choice of the corresponding $C_i(\ell)$. Thus the size of any DAG
  decomposition of width at most $n+s(n)-1$ is at least $(\log n/16
  )^{\log n/4}$. Recall that the size of $G_n(s,t)$ is polynomial in
  $n$ for $t(n)\le n$.


\end{proof}

\begin{corollary}
There is no polynomial size approximation of an optimal DAG
decomposition of $G_n(s,t) $ with an additive constant error. 
\end{corollary}


\subsection{\dagw is co-\np-hard}\label{sec:copnhard}

The construction of $G_n(s,t)$ shows how the robber can save the
history of the play in the current position. We extend it to prove
that the decision problem \DAGWprob (given a graph~$G$ and a
number~$k$, is $\DAGW(G)\le k$?) is co-\np-hard. For this we reduce
the \taut problem, which is co-\np-complete, to \DAGWprob. \taut is
the problem, given a formula of propositional logic, to decide whether
it is satisfied by all variable interpretations. Without loss of
generality, we may assume that the formula is given in CNF and no
variable appears in a clause twice. Let $\phi$ be a formula with~$n$
variables and $m$ clauses. The graphs $H_\phi$ are based on the graphs
$G_m(s,t)$ such that
\begin{itemize}
\item the number of levels in $G_m(s,t)$ is one plus the number~$n$ of
  variables in~$\phi$,

\item $s(\ell) = \lfloor \log \ell \rfloor$ and $t(\ell)=2$ for all levels~$\ell$.
\end{itemize}

It will be convenient to define functions that relate variables and levels.
Let the variables of $\phi$ be enumerated as $X_1$, $X_2$, \ldots, $X_n$. Let 
$\ell\colon \{1,\ldots,n\} \to \{5,6,\ldots,m\}$ be an injection that maps the 
index of a variable to a level. Let $v$ be the function mapping a level to an 
index of a variable such that $v(\ell) = i$ if and only if $\ell(i) = \ell$.

We replace $G_4(s,t)$ (which is a single vertex) by the following
gadget~$F_\phi$. It has a vertex $v$ and for every clause $C=L_1 \lor
L_2 \lor \ldots L_{r(C)}$ an $r(C)$-clique $K_C$ with vertices $v_1^C$,
$v_2^C$, \ldots, $v^C_{r(C)}$. The edges go from $v$ to every vertex of
$K_C$ and back, \ie we have edges $(v,v_i^C)$ and $(v_i^C,v)$ for all
clauses $C$ and all $i\in\{1,\ldots,r(C)\}$. From outside of $F_\phi$, all 
vertices that had
outgoing edges to the vertex of $G_4(s,t)$ now have outgoing
edges to all vertices of $F_\phi$. So those edges build the set $A^s(\ell)
\times F_\phi \cup N(\ell)\times F_\phi$ for every level~$\ell$. Finally, the edges from $K_C$
leaving $F_\phi$ reflect the clause~$C$. For all levels $\ell$ 
if $X_j$ with $j=v(\ell)$ does not appear in~$C$, then there are edges
$(v_j^C,b_0(\ell))$ and $(v_j^C,b_1(\ell))$. If $X_j = L_i$
for some~$i\in\{1,\ldots,r(C)\}$, then there is an edge $(v_j^C,b_1(\ell))$. If
$\neg X_{v(\ell)} = L_i$, then there is an edge $(v_i^C,b_0(\ell))$. 

We claim that $n+1$ cops capture the robber in $H_\phi$ if and only if
$\phi$ is a tautology. Whether $\phi$ is a tautology or not, the cops
can play according to the strategy as in the proof of
Lemma~\ref{lemma:dagw} until the robber component is $F_\phi$. They
also have to follow that strategy up to irrelevant changes as was
shown in Theorem~\ref{thm:super-poly}. In that position exactly one
cop is free (the one that would capture the robber on $G_4(s,t)$ if we
played on $G_n(s,t)$) and the others occupy all $A^s(\ell)$ (in all
levels) and, in each level $\ell$, one of the two vertices $b_0(\ell)$
and $b_1(\ell)$. The free cop is placed on $v$ in $F_\phi$ (there is
no other legal move that does not lead to an immediate loss for the cops) and 
the robber chooses some $K_C$ for a clause
$C=L_1 \lor L_2 \lor \ldots L_r$. Let $X_{j_i}$ be the variable in the 
literal $L_i$. Now for all levels $\ell$ all cops 
from all $A^s(\ell)$
cannot be removed and reused as this would violate the monotonicity:
there are edges from all vertices of $K_C$ to all vertices of all
$A^s(\ell)$. The cops from every level $\ell$ such that $X_{v(\ell)}$ does
not appear in $C$ cannot be removed for the same reason. If one cop
from some $B^t(\ell)$ can be reused, the cops win as
follows. Let this cop be in level $\ell$ and assume without loss of
generality that $v(\ell) = j_1$. The cop is placed on $v_2^C$, then the cop 
from $B^t(\ell(j_2))$ is placed on $v_3^C$. Now the cop from
$B^t(\ell(j_3))$ is placed on $v_4^C$ and so on.

Then the following holds.
 
\begin{lemma}\label{lemma:use_one_cop}
The cops can win if and
only if they can reuse one of~$r$ cops from those~$r$ levels~$\ell$
in which $X_{v(\ell)}$ appears in~$C$.
\end{lemma}

Assume that $\phi$ is true under every valuation. Let $R\subseteq
\{1,\ldots,n\}$ be the set of indices~$v(\ell)$ of $X_{v(\ell)}$ appearing in
$C$. Let $\alpha\colon \{X_i \mid i\in R\} \to \{0,1\}^r$ be the
valuation of those $X_{v(\ell)}$ defined by the choices of the robber
during the play as follows. For all levels~$\ell$, if 
$X_{v(\ell)}$
appears in $C$ and the robber chose the component $C_i(\ell)$ in level
$\ell$ (for $i\in\{0,1\}$), then $\alpha(X_{v(\ell)}) = 1$ if $i=0$ and
$\alpha(X_{v(\ell)}) = 0$ if $i=1$. Let $\beta$ be a valuation of
$X_1,\ldots,X_n$ extending $\alpha$. As $\beta \models \phi$,
$\beta\models C$ and thus there is some $L_j$ in $C$ with $\beta
\models L_j$. Let $\ell$ be such that $X_{v(\ell)} = L_j$ or $\neg X_{v(\ell)} =
L_j$ (we have $v(\ell)\in R$). If $X_{v(\ell)} = L_j$, then $\beta(X_{v(\ell)}) 
=
\alpha(X_{v(\ell)}) = 1$ and thus the robber chose $C_0(\ell)$ in
level~$\ell$. Then a cop occupies $b_0(\ell)$, but there is no edge
from $K_C$ to $b_0(\ell)$ (there is an edge to $b_1(\ell)$), so the
cop from $b_1(\ell)$ can be reused and the cops win. If $\neg X_{v(\ell)} =
L_j$, the situation is symmetric.

If $\phi$ is not a tautology, let $\beta$ be a valuation with $\beta
\not\models \phi$. The robber winning strategy is to choose in level
$\ell$ the component $C_1(\ell)$ if $\beta(X_{v(\ell)}) = 0$ and the component
$C_0(\ell)$ otherwise. When the cops occupy $v$, the robber chooses the
component $F_C$ corresponding a clause $C = L_1 \lor \ldots \lor L_r$
with $\beta \not \models C$. Then $\beta \not \models L_j$ for all
$j\in\{1,\ldots,r\}$. Thus every cop in all $B^t(\ell)$ is still
reachable from the robber component and the cops lose. By 
Lemma~\ref{lemma:use_one_cop}, the cops win.

\[P_j = Q_jX_j,\ldots,Q_rX_r
\psi(X_1/\beta(X_1),\ldots,X_{j-1}/\beta(X_{j-1}),X_j,\ldots,X_r)\]
where $X_\ell/\beta(X_\ell)$ means that we replace all occurrences of
$X_\ell$ in $\psi$ by $\beta(X_\ell)$. If $Q_j = \forall$, then $P_j$
is a position of the universal player, otherwise $P_j$ belongs to the
existential player. A next position depends on the choice of
$\beta(X_{j+1})\in\{0,1\}$ and has the form 
\[Q_{j+1}X_{j+1},\ldots,Q_rX_r
\psi(X_1/\beta(X_1),\ldots,X_j/\beta(X_j),X_{j+1},\ldots,X_r)\,.\]

The remaining positions of the game are of the form $(\theta,\beta)$
where $\theta$ is a subformula of~$\psi$ and $\beta$ is the valuation
of the variables as chosen in first part of the play. The second part
starts in position $(\psi,\beta)$.  If $\theta = \theta_1 \lor \theta_2$,
the existential player moves to $(\theta_1,\beta)$ or to $(\theta_2,\beta)$
and if $\theta = \theta_1 \land \theta_2$, then the universal player moves
to $(\theta_1,\beta)$ or to $(\theta_2,\beta)$. In positions
$(X_i,\beta)$, the existential player wins if $\beta(X_i) = 1$ and
loses of $\beta(X_i) = 0$. In positions $(\neg X_i,\beta)$, the
universal player wins if $\beta(X_i) = 1$ and loses if $\beta(X_i) =
0$. The formula is true if and only of the existential player has a
winning strategy in the game.

It is very well known that deciding whether a given quantified formula
is true is \pspace-complete. % If we restrict the quantifier alternation
% depth of the input formula, we obtain problems that are complete for
% the levels of the polynomial hierarchy:
% \begin{itemize}
% \item $\Sigma_0^p\QBF = \Pi_0^p\QBF$ is the set of all propositional formulae,
% \item $\Sigma_{i+1}^p\QBF = \exists X_1 \ldots \exists X_k \psi$ where
%   $\psi \in \Pi_i^p$,
% \item $\Pi_{i+1}^p\QBF = \forall X_1 \ldots \forall X_k \psi$ where
%   $\psi \in \Sigma_i^p$.
% \end{itemize}
% Hereby $\Sigma_i^p\QBF$ is complete for $\Sigma_i^p$ and $\Pi_i^p\QBF$
% is complete for $\Pi_i^p$. We now show that \DAGWprob is hard for
% every level of the polynomial hierarchy.

The rest of the section is devoted to proof of the following theorem.

\begin{theorem}
 \DAGWprob is \pspace-complete.
\end{theorem}
The easier part is to show that \DAGWprob is in \pspace. It suffices
to prove that any play in the cops and robber game has polynomial
length. Then deciding the winner of the game is in \aptime
(alternating \ptime) and thus in \pspace. If~$k$ cops have a winning
strategy on a graph, they also have a winning strategy that always
prescribes to place cops in a way that the space available for the
robber shrinks. We consider a version of the game where the cops have
to play in this manner. Then they win if and only if they win in at
most~$2n$ moves where~$n$ is the number of vertices of the graph. Thus
any play lasts at most $2n$ steps.

For the hardness we reduce \QBF to \DAGWprob. Let \[\phi = Q_1
X_1\ Q_2 X_2\ldots Q_r X_r\ \psi(X_1,\ldots,X_r)\] be a quantified
boolean formula. Our construction of the graph $S_\phi$ extends the
construction from Section~\ref{sec:copnhard}. For every universal
quantifier we add a new level as described in
Section~\ref{sec:copnhard}. For each existential quantifier we add a
level that is depicted in Figure~\ref{fig:existential}.


\begin{figure}
  \centering
  \begin{tikzpicture}
    \node[draw,circle,inner sep=5mm] (C_0) at (0,0){$M$};
    \node[gray] at (0,-0.4){$n-s(n)$};

    % \node[vertex] at (2,0){};
    %   \node at (2.5,0){$\cdots$};
    % \node[vertex] at (3,0){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (D) at 
(2.5,0){$D$};
       % \node at (3,0.5){$D$};
  \draw (C_0) -- (D);

    \node[draw,circle,inner sep=5mm] (C_1) at (3,-3){$C_0$};
    \node[gray] at (3,-3.4){$n-s(n)$};
      % \node at (4.5,-3){$\cdots$};
    \node[draw,circle,inner sep=5mm] (C_t) at (6,-3){$C_1$};
    \node[gray] at (6,-3.4){$n-s(n)$};
%   \draw[-slim] (C_0) to (C_1);
%   \draw[-slim] (C_0) to (C_t);
%   \draw[-slim] (D) to (C_1);
%   \draw[-slim] (D) to (C_t);
\node[vertex] (c_1) at (2,-1.5){};
\node at (1.8,-1.8){$c_0$};
\node[vertex] (c_t) at (5,-1.5){};
\node at (4.8,-1.8){$c_1$};

\draw[-slim] (C_0) to (c_1);
\draw[-slim] (c_1) to (C_1);
\draw[-slim] (D) to (c_1);

\draw[-slim] (C_0) to (c_t);
\draw[-slim] (c_t) to (C_t);
\draw[-slim] (D) to (c_t);



   \draw[-slim,bend right] (C_1) to (D);
   \draw[-slim,bend right] (C_t) to (D);

    % \node[vertex] at (-3.5,-2){};
    %   \node at (-3,-2){$\cdots$};
    % \node[vertex] at (-2.5,-2){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (A) at 
(-3,-2){$A$};
       % \node at (-4,-1.5){$A = \{a^1,\ldots,a^s\}$};
    \draw[-slim] (A) to (C_0);

  \node[vertex] (b_1) at (-4,-5){};
   % \node at (-3,-5){$\cdots$};
  \node[vertex] (b_t) at (-2,-5){};
    \node[draw,ellipse,minimum height=5mm,minimum width=30mm] (B) at
    (-3,-5){};
  \node at (-4.9,-5.5){$B = \{b_0,b_1\}$};
  \draw (B) to (A);
  \draw[-slim,bend left=40] (C_1) to (b_1);
  \draw[-slim,bend left=40] (C_t) to (b_t);

   \node[draw,rectangle,minimum width=20mm,minimum height=15mm]
   (G_n-3) at (0,-3){$G_{n-s(n)-1}(s,t)$};
   \draw[-slim] (C_0) to (G_n-3);
   \draw[-slim,bend right] (D) to (G_n-3);
   \draw            (A) to (G_n-3);
   \draw[-slim] (G_n-3) to (B);



  \end{tikzpicture}
  \caption{The construction of $G_n(s,t)$. Indices $\cdot(n)$ are omitted.}
  \label{fig:existential}
\end{figure}

If $\phi$ has no variables, then if $\phi$ is true, $S_\phi$ is a single 
vertex, and if $\phi$ is false, $S_\phi$ is a 2-clique. (So one cop wins if and 
only if $\phi$ is true.) Otherwise we start the construction of $S_\phi$ with 
$F_\psi$ and for $j=r,r-1,\ldots,1$ we construct graphs $S_\phi^j$ 
such that $S_\phi^1 = S_\phi$. Assume that $S_\phi^{j+1}$ is already 
constructed, then $S_\phi^j$ is the following graph. There are two cases. If 
$Q_j = \exists$, then the vertex set is 
\[V(S_\phi^j) = V_\exists(j) = V(S_\phi^{j+1}) \cupdot A(j) \cupdot B(j) \cupdot
C_0(j)\cupdot C_1(j) \cupdot N(n)\cupdot\{c_0(j),c_1(j)\}\,.\] 
Hereby $N(j) = M(j)\cupdot D(j)$ and $B(j)$ 
are as $N(j)$, $M(j)$, $D^s(j)$ and $B^t(j)$ in $G_n(s,t)$, \ie \[|B(j)| = 
|D(j)| = 2, |C_i(1)| = |M(1)| = 4, |C_i(k+1)| = |M(k+1)| = |M(k)| + 3\] for 
all $k\in\{2,\ldots,j\}$ and $i\in\{0,1\}$. Furthermore, $B(j) = 
\{b_0(j), b_1(j)\}$.

The set of edges is
\begin{align*}
                    E(S_\phi^j) & = E(S_\phi^{j+1}) \cup {N(n) \choose 2} \cup 
\bigcup_{i=0}^{1}
{C_i(n) \choose 2} \cup {A(n) \choose 2}\\
                     &\cup \bigcup_{i=0}^1 \Bigl( \bigl(N(n) \times  
\{c_i(n)\}\bigr) \cup
                     \bigl(\{c_i(n)\} \times C_i(n)\bigr)\\
                     & \hspace{3cm}\cup \bigl(C_i(n) \times D(n)
                     \bigr) \cup \bigl(C_i(n) \times
                     \{b_i(n)\}\bigr) \Bigr) \\
                    & \cup
                     \bigl(B(n) \times A(n)\bigr) \cup
                     \bigl(A(n) \times B(n) \bigr)\cup \bigl(A(n) \times 
M(n)\bigr)\\
                    & \cup \bigl(N(n) \times V(S_\phi^{j+1})\bigr) \cup 
\bigl(A(n)
                     \times V(S_\phi^{j+1})\bigr)\\
                    & \cup \bigl( V(S_\phi^{j+1})
                     \times A(n) \bigr) \cup E(j)\,.
\end{align*}
Hereby $E(j)$, the edges connecting $F_\psi$ to the new level are
defined as follows. Let $K_C = \{v_1^C,\ldots,v_{r(C)}^C\}$ be a
clique in $F_\psi$ corresponding to a clause $C = L_1\lor,\ldots,
L_r$. If $X_j = L_i$, then $(v_i^C,b_1(j))\in E(j)$. If $\neg X_j =
L_i$, then $(v_i^C,b_0(j))\in E(j)$. Otherwise (\ie if $X_j$ does not
appear in $C$) $\{(v_i^C,b_0(j)),(v_i^C,b_1(j))\}\subseteq E(j)$.

In the second case $Q_j = \forall$. Then $V(S_\phi(j)) = V_\forall(j) = 
V_\exists(j) \setminus \{c_0(j),c_1(j)\}$ and the edegs are defined as in 
$H_\phi$. The difference to a universal level is hence that the edges
from $N(n)$ to $C_i(n)$ are now subdivided by $c_i(\ell)$ for $i\in\{0,1\}$.

We are going to show that $r+1$ cops win on $S_\phi$ if and only if the 
existential player wins $\MCGAME(\phi)$. For that we need some 
lemmata.

Consider a positon $P$ in the game on $S_\phi$ in that there is a
level $\ell$ such that the robber is in $M(\ell)$. Let $b = (b_1,\ldots, b_r)$ 
be a tuple of bits and let $O^b(\ell) = \bigcup_{\ell'>\ell} A(\ell')\cup 
\{b_i(\ell') \mid b_1 = 1\}$. Assume that the cops occupy $O^b(\ell)$. Then the 
robber is
blocked in the levels less or equal to $\ell$ (except that he can go to some 
$b_i(\ell')$, but he would be captured there immediately). Assume that there
are $|N(\ell)|+1$ free cops in that position. 

\begin{lemma}\label{lemma:cops_invariant}
For each $i\in\{0,1\}$, the cops have a strategy that allows them either to
capture the robber or to expel him from level~$\ell$ such that the
cops occupy precisely $O^b(\ell)\cup A(\ell) \cup \{b_i(\ell)\}$ for an 
$i\in\{0,1\}$. 
\end{lemma}
\begin{proof}
The strategy is as follows. One cop is placed on $c_{1-i}(\ell)$. This
creates two components of $S_\phi^\ell$: the one induced by $C_0(\ell)$ and the one
induced by $N(\ell)$, $A(\ell)$, $B(\ell)$, $C_i(\ell)$ and
$S_\phi^{\ell-3}$. If the robber is in $C_i(\ell)$, the remaining free cops
expel him from there and the robber is in the other component. Then
the cops occupy $N(\ell)$ and then the cop from $c_{1-i}(\ell)$
occupies $b_i(\ell)$. If the robber is in $C_i(\ell)$ and stays there,
he is captured there by the cops from $N(\ell)$, so assume that the
robber goes either to the component induced by $b_{1-i}(\ell)$
or to
the component induced by $A(\ell)$ and $S_\phi^{\ell-3}$. In any case the
cops leave $D(\ell)$ and occupy $A(\ell)$. If the robber remains
in $b_{1-i}(\ell)$, he is captured by the cop from $b_i(\ell)$, so
assume that he goes to $S_\phi^{\ell-3}$. We obtain the required
position. 
\end{proof}

\begin{lemma}\label{lemma:robber_invariant}
The robber has a strategy that permits him either to
win or to reach a position from position $P$ where the robber is in
$S_\phi^{\ell-3}$ and the cops occupy $O^b(\ell)$, $A(\ell)$ and at least 
one of $b_i(\ell)$. Furthermore, this robber strategy is winning if
there are only $|M(\ell)|$ free cops.
\end{lemma}
\begin{proof}
The robber stays in $N(\ell)$ until it is completely occupied by the
cops. In that position, one of $c_i(\ell)$ is not occupied by cops,
and the robber runs to a $C_i(\ell)$ and plays as
in the proof of Theorem~\ref{thm:super-poly}. Note that the cops from $A(\ell')$ 
and from $B(\ell')$
for all $\ell'>\ell$ cannot be removed.
\end{proof}


\begin{lemma}
  There is a winning strategy for $r+1$ cops on $S_\phi$ if and only if
  $\phi$ is true.
\end{lemma}
\begin{proof}
  Assume that~$r$ cops have a winning strategy~$\sigma$
  on~$S_\phi$. In $\MCGAME(\phi)$, the
  existential player simulates the cops and robber game on $S_\phi$ by
  translating the moves of the existential player into robber moves
  and translating cop moves (according to~$\sigma$) into his choices
  of the existentially quantified variables. Assume that we reached a
  position~$P$ in the cops and robber game and a position $P_i$ (for
  $i\ge 1$) in the $\MCGAME(\phi)$ sich that the following invariant (INV) holds.
\begin{itemize}
 \item the values $b_j = \beta(X_j)$ for the variables $X_j$ where 
$j\in\{1,\ldots,i-1\}$ are already chosen,

\item in the cops and robber game, the robber is in level $\ell = 
\ell(i)$ and

\item the cops occupy $O^b(\ell)$ for the tuple $b =
  (b_1,\ldots,b_{i-1})$ where $O^b(\ell)$ is defined as above. 
\end{itemize}
Then there are exactly $\ell+1$ free cops. If $Q_i = \forall$, the
universal player chooses a value $b_i = \beta(X_i)$ for $X_i$. Then
the existential player simulates the cops and robber game playing for
the cops according to~$\sigma$ from position~$P$ and for the robber as in
Lemma~\ref{lemma:robber_invariant} such that the robber is expelled
from level $\ell$ and $A(\ell)$ and $b_i(\ell)$ are occupied by cops. The number of
free cops suffices for that. It is straightforeward to check that the
above invariant holds for $i+1$ and for the position of the cops and
robber game where the robber is blocked in the next level, \ie in level~$\ell-3$.

If $Q_i = \exists$, the existential player simulates the cops and robber 
game from~$P$ until the robber is expelled from level~$\ell$ according to 
Lemma~\ref{lemma:cops_invariant}. Hereby, the cops play according
to~$\sigma$ and the robber plays arbitrarily, but such that he is not
captured in level~$\ell$. For example, the robber goes directly to
$S_\phi^{\ell -3}$.  Again, there are enough free cops for 
the simulation. Then exactly one of $b_0(\ell)$ and $b_1(\ell)\}$ is opccupied 
by a cop. If it is $b_0(\ell)$, the existential player sets $\beta(X_i) = 0$, 
otherwise $\beta(X_i) = 1$. Again, the invariant holds.

When all variables have their values, the universal player chooses a
clause~$C$ and the universal player simulates in the cops and robber
game the move of the free cop to vertex~$v$ in $F_\psi$ and the move
of the robber to~$K_C$. As the cops have played according to~$\sigma$
and~$\sigma$ is a winning strategy, there is a free cop. The cops completely 
occupy all $A(\ell)$ and for all
$\ell$ exactly one of $b_0(\ell)$ and $b_1(\ell)$. Every vertex in all
$A(\ell)$ is still reachable from the robber vertex, so the free cop
is in some $b_i(\ell)$. As the cop is free, there is no edge from any
$v_j^C$ to $b_i(\ell)$, \ie there is the edge from some $v_j^C$ to
$b_{1-i}(\ell))$. By construction of $S_\phi$, $X_j$ appears
in~$C$ and if $i=0$, then $X_j$ is negativ and if $i=1$, then
$X_j$ is positiv in~$C$. In the first case $b_i = 0$ and
$\beta(X_{v(\ell)}) = 0$, so~$C$ is satisfied and the existential
player wins by choosing $\neg X_j$. The second case is
symmetric.

For the other direction assume that the existential player has a winning 
strategy. We show that~$r$ cops have a winning strategy. The cops simulate 
the game $\MCGAME(\phi)$ while playing on $S_\phi$ by translating he moves of 
the 
robber to choices of the universal player and the choices of the existential 
player to their moves. Assume as before that (INV) holds for
some~$i\ge 1$.

There are two cases: level~$\ell$ is either existential or universal. In any 
case, there are $\ell + 1$ free cops and if the level is universal,~$\ell$ of 
them occupy $N(\ell)$. The robber escapes to some $C_i(\ell)$ for an $i\in 
\{0,1\}$ or goes to the component consisting of $A(\ell)$, $B(\ell)$ and 
$S_\phi^{\ell-3}$. If the robber is in $C_i(\ell)$ the last remaining cop is 
placed on $b_i(\ell)$ and the robber proceeds to $\{b_{1-i}(\ell)\}\cup 
A(\ell) \cup S_\phi^{\ell-3}$, otherwise the cop is placed on 
$b_i(\ell) = b_0(\ell)$ and the robber is in $\{b_1(\ell)\}\cup A(\ell) \cup 
S_\phi^{\ell-3}$. Now the cops from $D(\ell)$ occupy $A(\ell)$ and the robber 
goes to $S_\phi^{\ell-3}$ (if he goes to the free vertex of $B(\ell)$, he loses 
immediately). Finally, the cops simulate the choice of the universal player: 
$\beta(X_{v(\ell)}) = i$. It is easy to see that the invariant holds.

If the level is existential, the cops look up what value the strategy for the 
existential player in $\MCGAME(\phi)$ prescribes to choose for 
$X_{v(\ell)}$: $\beta(X_{v(\ell)}) = b_i \in \{0,1\}$. Then according to 
Lemma~\ref{lemma:cops_invariant} the cops can play such that the invariant 
holds again.

When the play arrives $F_\psi$, there is one free cop that is placed on~$v$ and 
the robber goes to some $K_C$ for a clause~$C$. As the existential player has a 
winning strategy, there is some literal $L_j$ in~$C$ that is satisfied 
by~$\beta$. Without loss of generality, $L_j = X_i$ and $\beta(X_i) = 1$. Then 
$b_1(\ell(i))$ is occupied by a cop, but there is no edge from~$v_i^C$ to 
$b_1(\ell(i))$. Recall that in $C$ every variable appears at most once, so 
there is no edge from~$C$ to $b_1(\ell(i))$ and the cop from $b_1(\ell(i))$ is 
free.
\end{proof}


==> bigdec.tex <==
\section{Big DAG Decompositions}

Let $s,t\colon \bbN \to \bbN$ be two monotonically non-increasing
functions with $2\le s(n) < n/\log n$ and $2\le t(n)$ for
all~$n\ge5$. We define a class of graphs $G_n(s,t)$ of \dagw~$n+1$
such that every DAG decomposition of width $n+1$ has
super-polynomially many bags in the size of $G_n(s,t)$ (measured in
the number of vertices), which is in $O(n^2\cdot t(n)) = O(n^2\cdot t(n))$. The
parameter~$s$ will be used to determine the difference between the
optimal width of a DAG decomposition and the best possible width of a
polynomial size decomposition. The parameter~$t\ge 2$ is used for
fine-tuning. Our proof works already if $s(n) = t(n) = 2$ for all~$n$
and the reader is invited to assume these values at first. We shall
consider what changes if~$s$ and~$t$ are different later.

For $n\in\{1,\ldots,4\}$, the graph $G_1(s,t)$ is a single
vertex without edges. For $n\ge 5$, the graph $G_n(s,t)$ is
constructed as follows (see Figure~\ref{fig:graph}).  Let $M(n)$ and $C_i(n)$ for
$i\in\{0,\ldots,t(n)-1\}$ be pairwise disjoint sets of vertices, each of
$n-s(n)$ elements. Let $D^s(n)$ be a set of~$s(n)$ elements disjoint from
all $C_i(n)$ and $M(n)$, and let $N(n) = M(n) \cup D^s(n)$. Let $A^s(n)$ be a set
of~$s(n)$ new vertices, and let $B^t(n) = \{b_0(n),\ldots,b_{t(n)-1}(n)\}$ be a
set of~$t(n)$ new vertices.  The graph $G_n(s,t)$ has vertices
\[V(G_n(s,t)) = V(G_{n-s(n)-1}(s,t)) \cupdot A^s(n) \cupdot B^t(n) \cupdot
\bigcup_{i = 0}^{t(n)-1} C_i(n)\cupdot N(n)\,.\]
 We say that vertices from $A^s(n) \cup B^t(n) \cup \bigcup_{i = 0}^{t(n)-1} C_i(n) \cup N(n)$
are in level~$n$. For a set $X$ let $X \choose 2$ denote the set
$\{(x,y)\in X^2 \mid x\neq y\}$. The edges are defined by
\begin{align*}
E(G_n(s,t)) = &E(G_{n-s(n)-1}(s,t)) \cup {N(n) \choose 2} \cup \bigcup_{i=0}^{t(n)-1}
{C_i(n) \choose 2} \cup {A^s(n) \choose 2}\\
                     &\cup \bigcup_{i=0}^{t(n)-1} \Bigl( \bigl(N(n) \times
                     C_i(n)\bigr) \cup \bigl(C_i(n) \times D^s(n)
                     \bigr) \cup \bigl(C_i(n) \times
                     \{b_i(n)\}\bigr) \Bigr)\\
                    & \cup
                     \bigl(B^t(n) \times A^s(n)\bigr) \cup
                     \bigl(A^s(n) \times B^t(n) \bigr)\cup \bigl(A^s(n) \times M(n)\bigr)\\
                    & \cup \bigl(N(n) \times V(G_{n-s(n)-1}(s,t))\bigr) \cup \bigl(A^s(n)
                     \times V(G_{n-s(n)-1}(s,t))\bigr)\\
                    & \cup \bigl( V(G_{n-s(n)-1}(s,t))
                     \times A^s(n) \bigr) \cup \bigl(V(G_{n-s(n)-1}(s,t)) \times B^t(n)\bigr)\,.
\end{align*}
In other words, the first line says that $G_n(s,t)$ has all edges from
$G_{n-s(n)-1}(s,t)$, and that $N(n)$, all~$C_i(n)$
for $i\in\{0,\ldots,t(n)-1\}$ and $A^s(n)$ are cliques of sizes~$n$, $n-s(n)$
and~$s$, respectively. Note also that $B^t(n)$ induces an independent set.


\begin{figure}
  \centering
  \begin{tikzpicture}
    \node[draw,circle,inner sep=5mm] (C_0) at (0,0){$M$};
    \node[gray] at (0,-0.4){$n-s(n)$};

    % \node[vertex] at (2,0){};
    %   \node at (2.5,0){$\cdots$};
    % \node[vertex] at (3,0){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (D) at (2.5,0){$D^s$};
       % \node at (3,0.5){$D^s$};
  \draw (C_0) -- (D);

    \node[draw,circle,inner sep=5mm] (C_1) at (3,-3){$C_0$};
    \node[gray] at (3,-3.4){$n-s(n)$};
      \node at (5,-3){$\cdots$};
    \node[draw,circle,inner sep=2.6mm] (C_t) at (7,-3){$C_{t(n)-1}$};
    \node[gray] at (7,-3.4){$n-s(n)$};
   \draw[-slim] (C_0) to (C_1);
   \draw[-slim] (C_0) to (C_t);
   \draw[-slim] (D) to (C_1);
   \draw[-slim] (D) to (C_t);
   \draw[-slim,bend right] (C_1) to (D);
   \draw[-slim,bend right] (C_t) to (D);

    % \node[vertex] at (-3.5,-2){};
    %   \node at (-3,-2){$\cdots$};
    % \node[vertex] at (-2.5,-2){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (A) at (-3,-2){$A^s$};
       % \node at (-4,-1.5){$A^s = \{a^1,\ldots,a^s\}$};
    \draw[-slim] (A) to (C_0);

  \node[vertex] (b_1) at (-4,-5){};
    \node at (-3,-5){$\cdots$};
  \node[vertex] (b_t) at (-2,-5){};
    \node[draw,ellipse,minimum height=5mm,minimum width=30mm] (B) at
    (-3,-5){};
  \node at (-5.2,-5.5){$B^t = \{b_0,\ldots,b_{t(n)-1}\}$};
  \draw (B) to (A);
  \draw[-slim,bend left=40] (C_1) to (b_1);
  \draw[-slim,bend left=40] (C_t) to (b_t);

   \node[draw,rectangle,minimum width=20mm,minimum height=15mm]
   (G_n-3) at (0,-3){$G_{n-s(n)-1}(s,t)$};
   \draw[-slim] (C_0) to (G_n-3);
   \draw[-slim] (D) to (G_n-3);
   \draw            (A) to (G_n-3);
   \draw[-slim] (G_n-3) to (B);



  \end{tikzpicture}
  \caption{The construction of $G_n(s,t)$. Indices $\cdot(n)$ are omitted.}
  \label{fig:graph}
\end{figure}

For the following lemma the precise definition of~$s$ and $t$ in
$G_{n-s(n)-1}(s,t)$ is inessential.

\begin{lemma}
  \label{lemma:dagw}
The \dagw of $G_n(s,t)$ is $n+1$.
\end{lemma}
\begin{proof}
  The cops have the following winning strategy for the \dagw game on
  $G_n(s,t)$. First they occupy $N(n)$ and we can assume that the
  robber chooses some $C_i(n)$ (for $i\in\{0,\ldots,t(n)-1\}$) because all
  other strongly connected components of $G_n(s,t) - N(n)$ have
  incoming edges from all~$C_i(n)$. (So the robber can go
  to every other vertex that is reachable now also later, see Lemma~5.21
  in~\cite{RabinovichPhD}.)  Then the remaining cop occupies $b_i(n)$. If
  the robber stays in $C_i(n)$, the cops from $M(n)$ capture him there
  (recall that $M(n)$ has the same size $n-s(n)$ as every $C_i(n)$,
  $i\in\{0,\ldots,t(n)-1\}$). So we can assume that the robber goes to
  $A^s(n) \cup (B^t(n)\setminus\{b_i(n)\})$ (again, there is no reason for him 
to go directly to
  $G_{n-s(n)-1}(s,t)$). If the robber remains in $B^t(n)$, he is captured in 
the next move. The cops from $D^s(n)$ move to $A^s(n)$ and
  force the robber to proceed to $G_{n-s(n)-1}(s,t)$. From now on, the $s+1$
  cops in $A^s(n) \cup \{b_i(n)\}$ stay there until the end of the play
  and the remaining $n-s(n)$ cops play in $G_{n-s(n)-1}(s,t)$ in the same
  way as on $G_n(s,t)$ until the robber is captured or expelled to a
  $b_j(n)$ for $j\neq i$. There he will be captured in one move. Note
  that $G_{n-s(n)-1}(s,t)$ has outgoing edges only to $B^t(n)$ and to $A^s(n)$.

  A winning robber strategy against~$n$ cops is to stay in $N(n)$
  until all~$n$ cops are there and then to go to $C_0(n)$. In that
  position of the game, no cop can be removed from his vertex due to
  the monotonicity winning condition.
\end{proof}

We now prove that the described winning strategy for~$n+1$ cops (let
us call it~$\sigma$) is the only possible one up to some irrelevant
changes. Then we count the number of positions that are consistent
with~$\sigma$ and observe that there are super-polynomially many of
them. It will follow that every DAG decomposition of the optimal width
has a super-polynomial size.

The first kind of change is to occupy the sets $M(n)$, $C_i(n)$
($i\in\{0,\ldots,t(n)-1\}$), $A^s(n)$ and $D^s(n)$ in a different order
than according to~$\sigma$,
which, obviously, makes no sense, as~$\sigma$ prescribes to occupy
either the whole set or none of its vertices and those vertices have
ingoing and outgoing edges from and to the same vertices. The second
kind of a change is to place cops on and then to remove them from
vertices that are already unavailable for the robber. (Note
that~$\sigma$ never lets cops stay on such vertices.) This is also
useless because of the monotonicity. Both changes can obviously only
increase the number of possible positions.

\begin{lemma}\label{lemma:decs_and_positions}
If there is a DAG decomposition of a graph $G$ of width $k$ and of
size $n$, then $k$ cops have a winning strategy such that the number
of positions consistent with this strategy is at most~$n\cdot |G|$.
\end{lemma}
\begin{proof}
  Consider the strategy (let us call it $\sigma$) obtained from a DAG
  decomposition of width $k$ as described in \cite[Theorem
  16]{BerwangerDawHunKreObd12}. In a play consistent with~$\sigma$, the
  cops occupy only sets of vertices that correspond to some bag. Thus
  there are at most $n$ cop placements that can appear in a play. A
  position can be described by the cop placement and the robber
  vertex. There are at most $|G|$ vertices, so the total number of
  positions is at most $n\cdot |G|$.
\end{proof}


\begin{theorem}\label{thm:super-poly}
Every DAG decomposition of $G_n(s,t)$ of width $n+1$ has
super-po\-ly\-no\-mial\-ly many bags.
\end{theorem}
\begin{proof}
We describe the strategy of the robber that enforces the cops to play
according to~$\sigma$ up to irrelevant changes. If $n+1$ cops play in
a different way, they lose.

The robber remains in $N(n)$ until it is completely occupied by cops. If
a cop was placed on a vertex $v\notin N(n)$ before $N(n)$ was
completely occupied, the cops lose. Indeed, consider the position
where all vertices of $N(n)$ are occupied for the first
time. Because~$v$ (whatever it is) has been occupied and because it is
still reachable now from $N(n)$, the last $(n+1)$-st cop is still
on~$v$, otherwise the monotonicity is violated. The robber goes to
some $C_i(n)$ from which~$v$ is reachable via paths avoiding $N(n)$
(such a $C_i(n)$ always exists) and the cops have no legal move. Thus
the first moves of the cops are to occupy $N(n)$ and the last cop
remains outside of the graph.

The robber chooses some $C_i(n)$ and the cops have no other possible
move than to place the last remaining cop on $b_i(n)$ (otherwise we have the
situation discussed in the previous paragraph). The robber goes to
$A^s(n)\cup B^t(n)\setminus \{b_i(n)\}$. In this position, the cops in 
$\{b_i(n)\} \cup M(n)$ cannot
be removed and all $C_i(n)$ are unavailable for the cops. So the cops
from $D^s(n)$ must be used and they can be placed either in $A^s(n)$
or in $G_{n-s(n)-1}(s,t)$, or in $B^t(n)\setminus \{b_i(n)\}$. If at least one 
cop is placed in $G_{n-s(n)-1}(s,t)$ or in $B^t(n)\setminus \{b_i(n)\}$, the 
robber remains in $A^s(n)$ until all cops are
placed. Then the cops have no legal move and lose. It follows that the
cops must occupy the whole $A^s(n)$ and the robber goes to
$G_{n-s(n)-1}(s,t)$. From now on, all cops occupying $A^s(n)$ and
$b_i(n)$ will be reachable from the robber vertex and must stay
there. It follows by induction on~$n$ that~$\sigma$ is the unique
winning strategy for $n+1$ cops up to irrelevant changes.

We now count the number of positions that are consistent
with~$\sigma$. When the robber goes to the last level, the cops are
occupying $A^s(\ell)$ for all levels $\ell$ that appear as
indices of $G_\ell( s,t)$. Additionally, for each $\ell$, the cops
occupy exactly one of $\{b_0(\ell),\ldots,b_{t(\ell)}(\ell)\}$. (If they
occupy more of them, the remaining cops do not suffice to capture the
robber due to \Cref{lemma:dagw}.)  Thus when the robber is in the
lowest level of the recursion, there are $t^{\#\ell}$ positions where
$\#\ell$ is the total number of levels in the graph and $t = \min
\{t(\ell) \mid~\ell \text{ is a level in }G_n(s,t)\}$. As
$s(\ell)<\ell/\log \ell \le n\log n$, there are at least $\log n$
levels, \ie $\#\ell \ge \log n$ and the number of bags is at least
$t^{\log n}$. 

The size of $G_n(s,t)$ is 
\begin{align*}
|G_n(s,t)|& = |N(n)| + t(n)\cdot |C_i(n)| + |A^s(n)| +
|B^t(n)| + |G_{n-s(n)-1}(s,t)|  \\
&= n + t(n)\cdot (n-s(n)) + s(n) + t(n) + |G_{n-s(n)-1}(s,t)|
= O(n^2\cdot t(n))\,,
\end{align*}
 so $t^{\log n}$ is super-polynomial in
$|G_n(s,t)|$ for $\log n\le t\le n$.

Consider a DAG decomposition $\calD$ of $G_n(s,t)$ of width
$n+1$. Towards a contradiction assume that~$\calD$ has at most
$|G_n(s,t)|^c$ bags where~$c$ is a constant. Then the winning strategy
for $n+1$ cops induced by~$\calD$ has at most $|G_n(s,t)|^{c+1}$
positions. We have seen, however, that the number of positions consistent
with~$\sigma$ is super-polynomial in $G_n(s,t)$. 
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "bigDAGdecs"
%%% End: 


==> conclusion.tex <==
\section{Conclusion}
We showed that \dagw cannot be computed efficiently in the classical
sense (assuming \ptime${}\neq{}$\pspace).  It would be interesting to
find (fixed-parameter tractable) algorithms that compute reasonable
approximations of an optimal DAG decompositions. Another approach to
\dagw would be to show that \dagw and \kw are bounded in each other,
as deciding \kw is in \nptime. It is known that \dagw is
bounded in \kw by a quadratic function~\cite{KaiserKreRabSie14}.

Yet an other way to cope with the problem shown here is to weaken the power
of cops by forbidding them to be placed outside the robber
component. It is easy to see that in this case the DAG decomposition
resulting from a winning cop strategy (if they still can win) has size
polynomial in the size of the graph. That restriction also allows one to
solve the monotonicity cost problem: given a strategy for~$k$ cops
that guarantees a capture of the robber, how many cops are needed to
do this in a robber-monotone way? In the restricted version one can
come up  with a linear number of additional cops~\cite{KaiserKreRabSie14}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "bigDAGdecs"
%%% End: 


==> howordered.tex <==
%\section{How the widths are ordered}\label{sec:ordering}
\section{Comparing Width Measures with Respect to Generality}\label{sec:ordering}

In this section we compare directed width measures with respect to the
generality of classes of digraphs of bounded width. Besides the width
measures already mentioned we also consider \emph{D-width} and \emph{\Kw}.

\begin{figure}
\begin{center}
\begin{tikzpicture}

\node (dtw) at (0,0){dtw};
\node (rmdtw) at (0,-1){rmdtw};
\node (cmdtw) at (3,0){cmdtw};
\node (DAGw) at (6,0){DAG-w};
\node (Kw) at (9,0){K-w};
\node (Dw) at (6,-2){D-w};
% \node (DSw) at (6,-4){DS-w};


\node[rotate=90] (eq_dtw_rmdtw) at
(0,-0.5){$=$};


\node[] (dtw_lt_cmdtw) at (1.5,0) {{$<$}};

\node[] at (4.5,0)
{$<$};

\phantom{\node[rotate=90] at (6,0.5) {{$=$}};}

\node[] (dagw_le_kw) at (7.5,0) {{$\le$}};

\node[rotate=-45] (cmdtw_lt_dw) at (4.5,-1) {{$<$}};

% \node[,rotate=90]
% at (6,-3.5) {{$=$}};

\node[rotate=90] at (5.9,-1) {$<$};
\node[rotate=-90] (dagw_lt_dw) at (6.1,-1) {{$<$}};

\node[rotate=50] at (7.2,-1.05){$<$};
\node[rotate=50] (kw_lt_dw) at (7.05,-0.95){{$>$}};


\end{tikzpicture}
\end{center}
\caption{The relations between different measures. }
\label{fig:scheme}
\end{figure}

In~\cite{Safari05}, Safari suggests \dw as another structural
complexity measure. In our definition, \dw differs from Safari's
version, but only at most by the factor of $2$.
Let $G$ be
a graph.
  A \emph{D-decomposition} of $G$ is a pair $(T,(X_t)_{t\in V(T)})$
  where $T$ is a tree and $X_t \subseteq V(G)$ for all
  $t\in V(T)$ such that for all $v\in V(G)$ the set $\{ t\in V(T) \mid
  v\in X_t\}$ is non-empty and connected in $T$ and for every edge
  $e = \{s,t\}\in E(T)$ and every strongly connected component~$C$ of
  $G-(X_s\cap X_t)$, either $V(C)\subseteq \bigcup_{r\in V(T_s)} X_r$
  or $V(C)\subseteq \bigcup_{r\in V(T_t)} X_r$, where $T_s, T_t$ are
  the two components of $T-e$.  The width of $(T,(X_t))$ is
  $\max_{t\in V(T)} |X_t|$. The \emph{D-width} of $G$, $\DW(G)$, is
  the minimum of the widths of all D-decompositions of $G$.


\Kw is a complexity measure for directed graphs introduced by Hunter 
and Kreutzer in~\cite{HunterKre08}. \Kw is similar to \dagw and can be
defined by a decomposition, by a graph searching game and by an
elimination oder, similar to \tw. 

An \emph{elimination order}~$\elorder$ for a graph $G =
(V,E)$ is a linear order on~$V$. For a vertex~$v$ define $V_{\elorderg
  v} \coloneqq \{u\in V \mid v\elorder u\}$. The
\emph{support} of a vertex~$v$ with respect to~$\elorder$ is
\[\supp_{\elorder}(v) \coloneqq \{u\in V \mid v\elorder u \text{ and there is }
v'\in\Reach_{G-V_{\elorderg v}}(v)\text{ with }(v',u)\in E\}\,.\] The
\emph{width} of an elimination order~$\elorder$ is $\max_{v\in
  V}|\supp_{\elorder}(v)|$. The \emph{\kw} $\KW(G)$ of~$G$ is one plus the
minimum width of an elimination order of~$G$.

Hunter and Kreutzer conjecture
in~\cite[Conjecture~$30$]{HunterKre08} that \dagw and \kw bound each
other by a constant factor. More generally, the question is whether
there is a function~$f\colon \bbN\to\bbN$ such that, for every
graph~$G$, we have 
\begin{enumerate}[(1)]
\item $\DAGW(G) \le f\cdot\KW(G)$ and
\item $\KW(G) \le f\cdot \DAGW(G)$. 
\end{enumerate}
In~\cite{HunterKre08} it is shown
that if $\KW(G) = k$, then $2k-1$ cops have a (possibility
non-{}monotone) winning strategy~$\sigma$ in the \dagw game. We demonstrate
that~$\sigma$ is, in fact, weakly monotone, thus answering the first
question affirmatively.

\begin{theorem}\label{thm_kw_to_dagw}
If $\KW(G) = k+1$, then $\wmDAGW(G) \le 2k+1$.
\end{theorem}
\begin{proof}[Proof sketch]
Our proof follows the proof of Theorem~$20$
from~\cite{HunterKre08}, which shows that an elimination order of
width~$k$ induces a (possibly non-{}monotone) strategy for $2k+1$ cops
in the \dagw game. We show that the constructed
strategy is weakly monotone.
\end{proof}


\begin{theorem}\label{thm:ordering}
%  The following relations hold:
\begin{enumerate}[(i),noitemsep]
  \item For all graphs $G$, if $\KW(G) = k$, then $\DAGW(G) =
    \calO(k^2)$.\label{item:one}
  \item There is a class $\{G_n\mid n>2\}$ of graphs with $\dTW(G_n) \le
    4$ and $\DW(G_n)\ge n$. \label{item:two}
  \item There is a class of graphs $\{G_n\mid n>2\}$ such
    that~$\DAGW(G_n), \KW(G_n), \cmdTW (G_n)\le 4$ (and thus \dtw is
    bounded), but $\DW(G_n) \ge n$. \label{item:three}
  \item  For all graphs $G$, $\DW(G) \le \otwmeasure(G)$. \label{item:four}
  \item   There is a class of graphs $\{G_n\mid n>2\}$ with $\dTW(G_n) = 1$,
  $\DAGW(G_n) = \KW(G_n) = \DW(G_n) = 2$, and $\oTW(G_n) > n$. \label{item:five}
\end{enumerate}
\end{theorem}
\begin{proof}[Proof sketch]
  Part~\ref{item:one}: In \cite{HunterKre08} it was shown that if
  $\KW(G) = k$, then~$2k-1$ cops can capture a robber in the \dagw
  game, possibly in a non-monotone way. It is easy to see from the
  proof that the constructed strategy is weakly monotone, so the
  result follows.

Part~\ref{item:two}: It is easily seen that if $\DW(G) = k$, then~$k$ cops have
a cop-monotone winning strategy in the directed tree width game: the
cops just follow the tree and the strategy is cop-monotone because $\{ t\in V(T) \mid
  v\in X_t\}$ is connected in~$T$ for all $v\in V(G)$. The result
  follows from Theorem~\ref{thm_non_cop_mon}.
  
  Part~\ref{item:three}: A vertex $v$ can occur in several branches of
  the strategy tree for all the games: once because the robber
  occupies it (in a component~$A$) and once while the robber is in a
  different component~$B$, but the cops occupy~$v$ to close a
  ``bottleneck'' for the paths from the robber to the previous cop
  positions. Hereby the cops do not need to occupy~$v$ immediately
  after $A$ and~$B$ are separated from each other by the cops. In a
  D-decomposition, however, if~$v$ is in bags from different branches,
  it must also be contained in their common predecessors. If there are
  many such vertices~$v$, the width of the D-decomposition becomes
  large. This can be utilised to construct the graphs $G_n$.

  Let $T^d_\ell$ be the complete undirected tree of branching
  degree~$d$ and depth~$\ell$. Then $G_n$ consists of two vertex
  disjoint parts. One is a copy~$T$ of $T^n_{n+1}$ with additional
  edges forming the downward transitive closure. The other part,
  denoted by ~$T'$, is another copy of $T^n_{n+1}$, but the edges are
  now directed and oriented upwards. The parts are connected by edges
  going from a vertex~$v$ in $T$ to its copy~$v'$ in~$T'$ and
  from~$v'$ to the parent of~$v$ in~$T$ (if~$v$ is not the root). Now we transform the
  resulting graph by applying the following operation once on each
  vertex of~$T$ (except the root) in a top-down manner. The current
  vertex $v\in V(T)$ is replaced by~$n$ copies $v_1$, \ldots,
  $v_n$. Let~$w$ be the parent of~$v$. Then the edge $\{v,w\}$ is
  replaced by edges $\{v_i,w\}$, the edge $(v,v')$ by edges $(v_i,v')$
  and the edge $(u',v)$ be edges $(u',v_i)$ if $v'$ is the parent
  of~$u'$. Every $v_n$ is the root of a copy of the subtree of~$T$
  rooted at~$v$. 

  A cop- and robber-monotone winning strategy for~$4$ cops in the
  \dagw and in the \dtw game is to follow the robber down the tree~$T$
  and simultaneously down~$T'$. The strategy for the \kw game is
  similar. We show that no D-decomposition of small width exists. Any
  candidate for a small decomposition must roughly follow the tree~$T$
  (similarly as if we were looking for a tree decomposition for~$T$
  without the upward transitive closure). This means, when a
  vertex~$v$ appears in a bag of the decomposition tree for the first
  time counting from the root of the decomposition tree (and we call
  that bag, ``the bag of~$v$''), there are many direct successors
  of~$v$ that appear only in bags below. Let $v_1$ be such a
  successor. In order to block cycles from~$v_1$ via~$v_1'$ in~$T'$ to
  a predecessor of~$v$ and back to~$v_1$ with few cops, a vertex
  from~$T'$, say~$v_1'$, must occur in a bag containing~$v_1$. There
  are~$n$ such vertices~$v_i$ with edges to $v_1'$, so~$v_1'$ is in
  the bag of every~$v_i$ in~$T$. Then~$v_1'$ is also in the bag
  of~$v$. As there are~$n$ such~$v_1'$, they all are in the bag
  of~$v$, so the width of the D-decomposition is at least~$n$. See the
  appendix for details. Note that \dtw and \dw are already separated
  by~\ref{item:two}.
  
Part~\ref{item:four}: The proof is straightforward: an oriented tree
decomposition is a D-decomposition.

Part~\ref{item:five}: The graph $G_n$ is constructed inductively. Let $G_1^m$ be a single
  vertex. Then $G_{i+1}^m$ has a new root $r(G_{i+1}^m)$ with~$m$ successors 
$v_1,\dots,v_m$ connected by an undirected edge. Each such successor $v_i$ is the root 
$r(G_i^m)$ of a copy of $G_i^m$ and has outgoing cross edges to all leaves of the 
copies $G_i^m$ rooted at $v_j$ with $j<i$. Finally, $G_n = G_n^n$. 

The resulting graph is a tree with ordered siblings and additional
edges going from a vertex to the leaves of all subtrees rooted at
smaller siblings. In the \dagw game, the cops win by just playing down
the tree and following the robber to a new component if he uses the
cross edges. For the \kw game, the strategy is similar. The
D-decomposition is the usual tree decomposition of a tree, the cross
edges can be ignored. 

For the \otw, note that the tree decomposition underlying an oriented
tree decomposition of small width essentially repeats the structure of~$G_n$.
However, then an incoming cross edge enforces the orientation
downwards, a cross edge leaving the same subtree enforces the orientation upwards, so such a
oriented tree decomposition does not exist.
\end{proof}

We obtain the picture shown in Figure~\ref{fig:scheme} whereby $\dPW$
is \dpw, which is the least general width (Inequalities~(3)
and~(6)). \kw and \dpw can be characterised by similar
games~\cite{HunterKre08,Barat06} whereby the robber moves in the \kw
game are more restricted (the robber is allowed to move only if a cop
is about to occupy his vertex), which leads to the Inequality in~(3). The
same example that separates (undirected) \tw from (undirected)
\pw~\cite{KirousisPap86} can be ised to separate \kw from \dpw
establishing the strictness of~(3).  The same example separates also
\otw from \dpw establishing the strictness of~(6). The Inequality can
be proven straightforwardly. 

The most general width is \dtw. Between it and \dpw, \dagw and \kw,
and \dw and \otw build two chains. In the \dagw and in the \kw games,
cop free paths from the robber vertex to vertices previously visited
by the cops are forbidden, otherwise the robber wins. This condition
is reflected in the corresponding decompositions (that we do not
consider here).  In D-decompositions and oriented tree decompositions this
condition must not be fulfilled if there is no cop free path back. An
example class of graphs $G_n$ whose DAG- and \kw are large, but whose
\dtw, \dw and oriented \tw are small, is given
in~\cite{BerwangerDawHunKreObd12}. It is a undirected full binary tree
of height~$n$ with additional edges building the upward transitive
closure. The additional edges neither influence the obvious
D-decomposition, nor the same oriented decomposition with the
orientation always upwards. Also in the \dtw game, the cops process the
tree top-down regardless of the additional edges. However, the \dagw
is~$n$ and thus the \kw also grows with~$n$ by Part~\ref{item:one} of
Theorem~\ref{thm:ordering} (this is Inequality~(2) in the
picture). Thus we obtain one direction of (7)--(10), resp. The other
direction of~(7) and~(8) is Theorem~\ref{thm:ordering}\ref{item:three} and
the other direction of~(9) and~(10) is
Theorem~\ref{thm:ordering}\ref{item:five}.

The Inequality~(4) was proven in~\cite{Safari05}, the strictness
is~Theorem~\ref{thm:ordering}\ref{item:two}. The Inequality~(5)
is~Theorem~\ref{thm:ordering}\ref{item:four}, the strictness is
Theorem~\ref{thm:ordering}\ref{item:five}.

The only blank spot in Figure~\ref{fig:scheme} is the strictness
of~(2), \ie whether \kw is a function of \dagw. It was conjectured
that \kw and \dagw differ by at most a constant
factor~\cite[Conjecture~$30$]{HunterKre08}. However, methods we used
in Theorem~\ref{thm:ordering}\ref{item:one} to show a weaker version
of one direction of the conjecture do not seem to apply for the other direction.

%  (1), (3),
% (6) and, essentially, $\DW, \oTW \lneq \DAGW, \KW$ (in (7), (8), (9)
% and (10), \ie that the latter two are not bounded in the former two)
% are proven in~\cite{BerwangerDawHunKreObd12}; ``$\le$'' in~(4) is
% proven in~\cite{Safari05}; the remaining statements are proven in
% Theorem~\ref{thm:ordering}: (2) is~\ref{item:one}; the strictness
% in~(4) and the other directions in (7) and (8) are~\ref{item:three};
% ``$\le$" in~(5) is~\ref{item:four}; the strictness in~(5) and
% $\DAGW,\KW \lneq \oTW$ (in (9) and~(10)) are~\ref{item:five}.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> intro.tex <==
\section{Introduction}

In the study of hard algorithmic problems on graphs,
methods derived from structural graph theory have proved to be a
valuable tool. The rich theory of special classes of graphs developed
in this area has been used to identify classes of graphs, such as
classes of bounded tree width or clique width,
on which many computationally hard problems can be solved
efficiently. 
Most of these classes are defined by some structural
property, such as having a tree decomposition of low width, and this structural 
information can be exploited
algorithmically. 

Structural parameters such as tree width, clique width, classes of graphs
defined by excluded minors etc.\@ studied in this context relate to
undirected graphs.
However, in various applications in computer science, directed graphs are
a more natural model. 
Given the enormous success
width parameters 
had for problems defined on undirected graphs, it is natural to ask
whether they can also be used to analyse the complexity of hard
algorithmic problems
on digraphs.
While in principle it is 
possible to apply the structure theory for undirected graphs to directed
graphs by ignoring the direction of edges, this implies a significant
information loss. Hence,
for computational problems whose instances are directed graphs,  
methods based on the structure theory for undirected graphs may be
less useful.

\Tw is one of the most successful structural complexity measures. It has several
characterisations coming from seemingly unrelated notions, \eg by
eliminations orders or cops and robber games. \Tw is also deeply
connected to graph minors and has numerous algorithmic applications.
The result of several approaches to generalise \tw to digraphs was a
number of structural complexity measures for digraphs. 
Reed \cite{Reed99} and Johnson, Robertson, Seymour and
Thomas~\cite{JohnsonRobSeyTho01} introduced the
concept of \emph{directed tree width} and showed that the $k$-disjoint
paths problem and more general linkage problems can be solved in
polynomial-time on classes of digraphs of bounded directed
tree width. Following this initial proposal, several alternative
notions of width measures for sparse classes of digraphs have been
presented, for instance \emph{directed path width} (see
\cite{Barat06}, initially proposed by Robertson, Seymour and Thomas),
\emph{D-width}~\cite{Safari05},
\emph{DAG-width}~\cite{BerwangerDawHunKreObd12} and
\emph{Kelly-width}~\cite{HunterKre08}. 

In this work we concentrate on \dagw. It distinguishes itself in its
particularly simple definition. DAG decompositions have a clear
structure and the definition of the cops and robber games
characterising \dagw is a straight forward and natural generalisation
of the corresponding game for \tw. However, we show some disadvantages
of \dagw.


% In this game corresponding to tree width, the searchers, often called \emph{cops}, reside on
% vertices of an undirected graph a$G$ nd so does the fugitive, often called
% the \emph{robber}. The game is played in rounds. Initially, there is
% no cop on the graph and the robber is free to choose a vertex
% $r$. This defines the first position $(\emptyset, r)$. In
% every round, where the cops are on a set $C$ of vertices and the
% robber is on a vertex $r$, the cops first announce their new position
% $C'$. The robber, knowing this choice, can then move to any other
% vertex in the graph reachable from his current position $r$ by a path
% in $G-(C\cap C')$. The cops win if at some point the robber cannot
% move anymore and his current position is also occupied by a
% cop. Otherwise, i.e. if the play is infinite, the robber wins. Clearly
% the cops can always win on any graph by placing a cop every
% vertex. Hence, the minimal number of cops required to catch the robber
% is a natural graph invariant for undirected graphs and it turns out
% that this number is exactly the tree width of $G$ (plus $1$) (see \cite{SeymourTho93}).

% Other variants of graph searching games are obtained by changing the
% rules of the game in various ways. For instance, the robber can be
% invisible and the cops have to move independent of his current
% position (which yields a game equivalent to path width), the robber
% may in addition only be allowed to move when a cops is to be placed on his current
% position (this is called inertness and also yields tree width), the robber may instead hide in edges (which is
% the original definition), the cops and
% the robber may only be allowed to move along a single edge rather than
% paths of any length and many further variants. Especially the last 
% variation leads to a very different type of graph searching games, 
% with a huge body of literature studying such games. In this paper we
% will not consider such games. 

A crucial task in designing efficient algorithms on graphs where some
width is bounded is to find a decomposition of the given graph of
small width. Such decompositions, usually trees or DAGs, are used to
solve the problem recursively following the decomposition. For \tw and
\dtw one can decompose the graph in fixed parameter tractable
time. For \dw and for \kw such algorithms are not known, but there is
always a decomposition of polynomial size, so it can be found non-deterministically. 
Only the complexity of \dagw was left as an open problem
as it was not known whether every digraph has a decomposition of
polynomial size.

Surprisingly, in this paper we show that deciding the \dagw of a
digraph is not only not in \np (under standard complexity theoretical
assumptions), it is in fact \pspace-complete. In terms of the \dagw
game this exhibits the worst case complexity of such games. This
result is quite unexpected and especially surprising as such a high
complexity was to date only exhibited by a form of graph searching
games called \emph{domination games} (see
\cite{FominKM03,FominGT11,KreutzerOrd09}). In these games, each cop
not only occupies his current vertex (as in other such games) but a whole neighbourhood of
fixed radius, which essentially allows to simulate set quantification
making the problem \pspace-complete.
The \dagw game, however, is to the best of our
knowledge the only graph searching game with the usual
capturing condition that exhibits such a complexity.

With the same proof technique we also show that there are classes of
graphs for which any DAG decomposition of optimal width must contain a
super-polynomial number of bags. (If \np${}\not={}$\pspace, this would
follow from the previous result, but we show this unconditionally.)
Furthermore, we obtain that there cannot be a polynomial time
approximation algorithm for \dagw with only an additive error.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "bigDAGdecs"
%%% End: 



==> prelim.tex <==
\section{Preliminaries}
\label{sec:prelims}

We assume familiarity with basic concepts of graph theory and refer
to~\cite{Diestel12} for background.  All graphs in this paper are
finite, directed and simple, i.e.~they do not have loops or multiple
edges between the same pair of vertices. Undirected graphs are
directed graphs with a symmetric edge relation.  If~$G$ is a graph,
then $V(G)$ is its set of vertices and $E(G)$ is its set of edges. For
a set $X\subseteq V(G)$ we write $G[X]$ for the subgraph of~$G$
induced by~$X$ and $G-X$ for $G[V(G)\setminus X]$. If $X$ is a set of
vertices, we write $\Reach_{G}(X)$ to denote the set of vertices
reachable from a vertex in~$X$. If $X=\{v\}$, we write $\Reach_G(v)$.
A strongly connected component of a digraph~$G$ is a maximal
subgraph~$C$ of~$G$ which is strongly connected, \ie~between any pair
$u,v\in V(C)$ there are directed paths from~$u$ to~$v$ and from~$v$
to~$u$. All components considered in this paper will be strong and
hence we simply write \emph{component}.  

A \emph{DAG decomposition} of~$G$ is a tuple $(D, B)$ where $D$ is a DAG and $B 
= \{B_d \mid d\in V(D)\}$ is a set of bags, \ie subsets of $V(G)$, such that
\begin{enumerate}
\item $\bigcup_{d\in V(D)} B_d = V(G)$,

\item for all $a,b,c \in D$, if $a < b < c$, then $B_a \cap B_c \subseteq B_b$,

\item for every root $r \in V(D)$, $\Reach_{G}(B_{\ge r}) = B_{\ge r}$
  where $B_{\ge r} = \bigcup_{r\le d} B_d$,

\item for each $(a,b)\in E(D)$, $\Reach_{G - (B_a \cap B_b)}(B_{\ge b}
  \setminus B_a) = B_{\ge b} \setminus B_a$.
\end{enumerate}
The width of $(D, B)$ is $\max_{d\in V(D)} |B_d|$ and its size is $|V(D)|$. The 
\emph{DAG-width} $\DAGW(G)$ of $G$ is the
minimal width of a DAG decomposition of~$G$.

\Dagw can be characterised by a cops and robber game. played 
on a graph $G$ by a team of cops and a robber. The
robber and each cop occupy a vertex of $G$. Hence, a current game
position can be described by a pair $(C, v)$, where $C$ is the set of
vertices occupied by cops and $v$ is the current robber position. At
the beginning the robber chooses an arbitrary vertex $v$ and the game
starts at position $(\emptyset, v)$. The game is played in rounds. In
each round, from a position $(C, v)$ the cops first announce their
next move, \ie~the set $C'\subseteq V(G)$ of vertices that they will
occupy next. Based on the triple $(C, C', v)$ the robber chooses his
new vertex $v'$. This completes a round and the play continues at
position $(C', v')$.  As we will see, from all positions $(C, C', v)$, \ie~when
the cops move from their current position $C$ to $C'$ and the robber
is on $v$, the robber has exactly the same choice of
moves from any vertex in the component of $G-C$ containing~$v$.  We
will therefore describe game positions by a pair $(C, R)$, or a triple
$(C, C', R)$, where $C, C'$ are as before and~$R$ induces a component of
$G-C$. 

Formally, a game is a tuple $(V,V_0,E,v_0,\Omega)$ where $(V,E)$ is a
directed graph, in which $V$ denotes the set of all positions and $E$
the set of moves, $V_0 \subseteq V$ is the set of positions in which
player~0 has to move, $v_0\in V$ is the start position and $\Omega\in
V^\omega$ is the winning condition. A play is a sequence $v_0$,
$v_1$,\ldots such that for all~$i\ge 0$, $(v_i,v_{i+1})\in
E$. Player~0 wins a play $\pi$ if it is finite and ends in a vertex
$v\in V_1\coloneqq V\setminus V_0$ without successors (so Player~1 has
to move, but cannot do this) or $\pi\in\Omega$. A (memoryless)
strategy for Player~0 is a partial function $\sigma\colon V\to V$ such
that for all $v\in V$ where $\sigma$ is defined, $(v,\sigma(v))\in
E$. Strategies for Player~1 are defined analogously. A play $v_0,
v_1,\ldots$ is consistent with $\sigma$ if for each $v_i\in V_0$ that
has a successor, we have $\sigma(v_i) = v_{i+1}$. We say that~$\sigma$
is winning if every play consistent with~$\sigma$ is winning for
Player~0 (and analogously for Player~1). We say that a game position
is consistent with~$\sigma$ if there is a play consistent
with~$\sigma$ which contains the position.


The \emph{\dagw game} $\DAGWgame{G} = (V,V_0,E,v_0,\Omega)$ on a
graph~$G$ is defined as follows. The set of positions is $V = \Pos(G)
= \Pos_c \cupdot \Pos_r $ where 
\[\Pos_c = V_0 =  \{(C,R) \mid C\subseteq V(G),  R\subseteq V(G) 
\text{ is a component of }G- C\}\] 
are cop positions and 
\[\Pos_r = \{(C,C',R) \mid C, C' \subseteq V(G) \text{ and }R\subseteq
V(G) \text{ is a component of }G-C\}\]
are robber positions. The set of moves is
$\Moves(G) = \Moves_c(G) \cupdot \Moves_r(G)$ where 
\[\Moves_c(G) \coloneqq \{\bigl( (C,R), (C,C',R) \bigr) \mid (C,R)\in \Pos_c,
(C,C',R)\in \Pos_r\}\]
are cop moves and 
\begin{align*}
\Moves_r(G) \coloneqq &\{\bigl( (C,C',R),(C',R') \bigr) \mid (C,C',R)\in \Pos_r, (C',R')\in
\Pos_c \\&\text{ and } R'\text{ is a component of } G-C' \text{ with
}R'\subseteq \Reach_{G-(C\cap C')}(R)\}
\end{align*}
are robber moves. The start
position is $(\0,\0,\0)$ and the winning condition for the cops (\ie
for Player~0) is $\Omega = \mathrm{Fin} \cap \Mon$ where
$\mathrm{Fin}$ is the set of all finite plays and $\Mon$ defines the
monotonicity condition as $\Mon \coloneqq
\{(C_0,C_1,R_0),(C_1,R_1),(C_1,C_2,R_1),\ldots\} \mid R_i\subseteq
R_{i+1} \text{ for all }i\ge 0$. In other words, the cops all finite
plays in which the robber could never visit a vertex that has already
been unavailable for him. All other plays are won by the robber.

A cop is \emph{free} in a position $(C,R)$ if he is outside of the
graph (\ie $|C|<k$ in the game with $k$ cops) or on 
a vertex $v\in C$ such that $v\notin \Reach_{G-(C\setminus \{v\})}(R)$, \ie 
removing this cop does not lead to non-robber-monotonicity.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "bigDAGdecs"
%%% End: 


==> pspace.tex <==
\section{\dagw is \pspace-complete}
\label{sec:pspace}

We extend our construction again to model choices of the cops in a
play that are still recognisable at the end of the play. This leads to
a reduction from \QBF, which is \pspace-complete, to
\DAGWprob. A \emph{quantified boolean formula} $\phi$ is of the form
$\phi = Q_1X_1\ldots Q_rX_r \psi(X_1,\ldots,X_r)$ where $Q_i$ is
either $\forall$ or $\exists$ and $\psi$ is a propositional formula in
CNF with variables from $\calX  =\{X_1,\ldots, X_r\}$. 

The semantics of $\phi$ can be defined by means of a two-player game
with perfect information, which is convenient for our reduction. It is
the model-checking game $\MCGAME(\phi)$ for $\phi$ on the fixed structure
$(\{0,1\},\0)$ with no relations. The
players are called $\forall$ (the universal player) and $\exists$ (the
existential player). A play is played as follows. First, the
quantifying prefix of the formula is read from left to right and, for
$i=1,2,\ldots,r$, player $Q_i\in\{\forall, \exists\}$ chooses a value
$\beta(X_i) \in\{0,1\}$ for $X_i$. In other words, we have
positions~$P_j$ of the form
\[P_j = Q_jX_j,\ldots,Q_rX_r
\psi(X_1/\beta(X_1),\ldots,X_{j-1}/\beta(X_{j-1}),X_j,\ldots,X_r)\]
where $X_\ell/\beta(X_\ell)$ means that we replace all occurrences of
$X_\ell$ in $\psi$ by $\beta(X_\ell)$. If $Q_j = \forall$, then $P_j$
is a position of the universal player, otherwise $P_j$ belongs to the
existential player. A next position depends on the choice of
$\beta(X_{j+1})\in\{0,1\}$ and has the form 
\[Q_{j+1}X_{j+1},\ldots,Q_rX_r
\psi(X_1/\beta(X_1),\ldots,X_j/\beta(X_j),X_{j+1},\ldots,X_r)\,.\]

The remaining positions of the game are of the form $(\theta,\beta)$
where $\theta$ is a subformula of~$\psi$ and $\beta$ is the valuation
of the variables as chosen in first part of the play. The second part
starts in position $(\psi,\beta)$.  If $\theta = \theta_1 \lor \theta_2$,
the existential player moves to $(\theta_1,\beta)$ or to $(\theta_2,\beta)$
and if $\theta = \theta_1 \land \theta_2$, then the universal player moves
to $(\theta_1,\beta)$ or to $(\theta_2,\beta)$. In positions
$(X_i,\beta)$, the existential player wins if $\beta(X_i) = 1$ and
loses of $\beta(X_i) = 0$. In positions $(\neg X_i,\beta)$, the
universal player wins if $\beta(X_i) = 1$ and loses if $\beta(X_i) =
0$. The formula is true if and only of the existential player has a
winning strategy in the game.

It is very well known that deciding whether a given quantified formula
is true is \pspace-complete. % If we restrict the quantifier alternation
% depth of the input formula, we obtain problems that are complete for
% the levels of the polynomial hierarchy:
% \begin{itemize}
% \item $\Sigma_0^p\QBF = \Pi_0^p\QBF$ is the set of all propositional formulae,
% \item $\Sigma_{i+1}^p\QBF = \exists X_1 \ldots \exists X_k \psi$ where
%   $\psi \in \Pi_i^p$,
% \item $\Pi_{i+1}^p\QBF = \forall X_1 \ldots \forall X_k \psi$ where
%   $\psi \in \Sigma_i^p$.
% \end{itemize}
% Hereby $\Sigma_i^p\QBF$ is complete for $\Sigma_i^p$ and $\Pi_i^p\QBF$
% is complete for $\Pi_i^p$. We now show that \DAGWprob is hard for
% every level of the polynomial hierarchy.

The rest of the section is devoted to proof of the following theorem.

\begin{theorem}
 \DAGWprob is \pspace-complete.
\end{theorem}
The easier part is to show that \DAGWprob is in \pspace. It suffices
to prove that any play in the cops and robber game has polynomial
length. Then deciding the winner of the game is in \aptime
(alternating \ptime) and thus in \pspace. If~$k$ cops have a winning
strategy on a graph, they also have a winning strategy that always
prescribes to place cops in a way that the space available for the
robber shrinks. We consider a version of the game where the cops have
to play in this manner. Then they win if and only if they win in at
most~$2n$ moves where~$n$ is the number of vertices of the graph. Thus
any play lasts at most $2n$ steps.

For the hardness we reduce \QBF to \DAGWprob. Let \[\phi = Q_1
X_1\ Q_2 X_2\ldots Q_r X_r\ \psi(X_1,\ldots,X_r)\] be a quantified
boolean formula. Our construction of the graph $S_\phi$ extends the
construction from Section~\ref{sec:copnhard}. For every universal
quantifier we add a new level as described in
Section~\ref{sec:copnhard}. For each existential quantifier we add a
level that is depicted in Figure~\ref{fig:existential}.


\begin{figure}
  \centering
  \begin{tikzpicture}
    \node[draw,circle,inner sep=5mm] (C_0) at (0,0){$M$};
    \node[gray] at (0,-0.4){$n-s(n)$};

    % \node[vertex] at (2,0){};
    %   \node at (2.5,0){$\cdots$};
    % \node[vertex] at (3,0){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (D) at 
(2.5,0){$D$};
       % \node at (3,0.5){$D$};
  \draw (C_0) -- (D);

    \node[draw,circle,inner sep=5mm] (C_1) at (3,-3){$C_0$};
    \node[gray] at (3,-3.4){$n-s(n)$};
      % \node at (4.5,-3){$\cdots$};
    \node[draw,circle,inner sep=5mm] (C_t) at (6,-3){$C_1$};
    \node[gray] at (6,-3.4){$n-s(n)$};
%   \draw[-slim] (C_0) to (C_1);
%   \draw[-slim] (C_0) to (C_t);
%   \draw[-slim] (D) to (C_1);
%   \draw[-slim] (D) to (C_t);
\node[vertex] (c_1) at (2,-1.5){};
\node at (1.8,-1.8){$c_0$};
\node[vertex] (c_t) at (5,-1.5){};
\node at (4.8,-1.8){$c_1$};

\draw[-slim] (C_0) to (c_1);
\draw[-slim] (c_1) to (C_1);
\draw[-slim] (D) to (c_1);

\draw[-slim] (C_0) to (c_t);
\draw[-slim] (c_t) to (C_t);
\draw[-slim] (D) to (c_t);



   \draw[-slim,bend right] (C_1) to (D);
   \draw[-slim,bend right] (C_t) to (D);

    % \node[vertex] at (-3.5,-2){};
    %   \node at (-3,-2){$\cdots$};
    % \node[vertex] at (-2.5,-2){};
    \node[draw,circle,minimum height=5mm,minimum width=10mm] (A) at 
(-3,-2){$A$};
       % \node at (-4,-1.5){$A = \{a^1,\ldots,a^s\}$};
    \draw[-slim] (A) to (C_0);

  \node[vertex] (b_1) at (-4,-5){};
   % \node at (-3,-5){$\cdots$};
  \node[vertex] (b_t) at (-2,-5){};
    \node[draw,ellipse,minimum height=5mm,minimum width=30mm] (B) at
    (-3,-5){};
  \node at (-4.9,-5.5){$B = \{b_0,b_1\}$};
  \draw (B) to (A);
  \draw[-slim,bend left=40] (C_1) to (b_1);
  \draw[-slim,bend left=40] (C_t) to (b_t);

   \node[draw,rectangle,minimum width=20mm,minimum height=15mm]
   (G_n-3) at (0,-3){$G_{n-s(n)-1}(s,t)$};
   \draw[-slim] (C_0) to (G_n-3);
   \draw[-slim,bend right] (D) to (G_n-3);
   \draw            (A) to (G_n-3);
   \draw[-slim] (G_n-3) to (B);



  \end{tikzpicture}
  \caption{The construction of $G_n(s,t)$. Indices $\cdot(n)$ are omitted.}
  \label{fig:existential}
\end{figure}

If $\phi$ has no variables, then if $\phi$ is true, $S_\phi$ is a single 
vertex, and if $\phi$ is false, $S_\phi$ is a 2-clique. (So one cop wins if and 
only if $\phi$ is true.) Otherwise we start the construction of $S_\phi$ with 
$F_\psi$ and for $j=r,r-1,\ldots,1$ we construct graphs $S_\phi^j$ 
such that $S_\phi^1 = S_\phi$. Assume that $S_\phi^{j+1}$ is already 
constructed, then $S_\phi^j$ is the following graph. There are two cases. If 
$Q_j = \exists$, then the vertex set is 
\[V(S_\phi^j) = V_\exists(j) = V(S_\phi^{j+1}) \cupdot A(j) \cupdot B(j) \cupdot
C_0(j)\cupdot C_1(j) \cupdot N(n)\cupdot\{c_0(j),c_1(j)\}\,.\] 
Hereby $N(j) = M(j)\cupdot D(j)$ and $B(j)$ 
are as $N(j)$, $M(j)$, $D^s(j)$ and $B^t(j)$ in $G_n(s,t)$, \ie \[|B(j)| = 
|D(j)| = 2, |C_i(1)| = |M(1)| = 4, |C_i(k+1)| = |M(k+1)| = |M(k)| + 3\] for 
all $k\in\{2,\ldots,j\}$ and $i\in\{0,1\}$. Furthermore, $B(j) = 
\{b_0(j), b_1(j)\}$.

The set of edges is
\begin{align*}
                    E(S_\phi^j) & = E(S_\phi^{j+1}) \cup {N(n) \choose 2} \cup 
\bigcup_{i=0}^{1}
{C_i(n) \choose 2} \cup {A(n) \choose 2}\\
                     &\cup \bigcup_{i=0}^1 \Bigl( \bigl(N(n) \times  
\{c_i(n)\}\bigr) \cup
                     \bigl(\{c_i(n)\} \times C_i(n)\bigr)\\
                     & \hspace{3cm}\cup \bigl(C_i(n) \times D(n)
                     \bigr) \cup \bigl(C_i(n) \times
                     \{b_i(n)\}\bigr) \Bigr) \\
                    & \cup
                     \bigl(B(n) \times A(n)\bigr) \cup
                     \bigl(A(n) \times B(n) \bigr)\cup \bigl(A(n) \times 
M(n)\bigr)\\
                    & \cup \bigl(N(n) \times V(S_\phi^{j+1})\bigr) \cup 
\bigl(A(n)
                     \times V(S_\phi^{j+1})\bigr)\\
                    & \cup \bigl( V(S_\phi^{j+1})
                     \times A(n) \bigr) \cup E(j)\,.
\end{align*}
Hereby $E(j)$, the edges connecting $F_\psi$ to the new level are
defined as follows. Let $K_C = \{v_1^C,\ldots,v_{r(C)}^C\}$ be a
clique in $F_\psi$ corresponding to a clause $C = L_1\lor,\ldots,
L_r$. If $X_j = L_i$, then $(v_i^C,b_1(j))\in E(j)$. If $\neg X_j =
L_i$, then $(v_i^C,b_0(j))\in E(j)$. Otherwise (\ie if $X_j$ does not
appear in $C$) $\{(v_i^C,b_0(j)),(v_i^C,b_1(j))\}\subseteq E(j)$.

In the second case $Q_j = \forall$. Then $V(S_\phi(j)) = V_\forall(j) = 
V_\exists(j) \setminus \{c_0(j),c_1(j)\}$ and the edegs are defined as in 
$H_\phi$. The difference to a universal level is hence that the edges
from $N(n)$ to $C_i(n)$ are now subdivided by $c_i(\ell)$ for $i\in\{0,1\}$.

We are going to show that $r+1$ cops win on $S_\phi$ if and only if the 
existential player wins $\MCGAME(\phi)$. For that we need some 
lemmata.

Consider a positon $P$ in the game on $S_\phi$ in that there is a
level $\ell$ such that the robber is in $M(\ell)$. Let $b = (b_1,\ldots, b_r)$ 
be a tuple of bits and let $O^b(\ell) = \bigcup_{\ell'>\ell} A(\ell')\cup 
\{b_i(\ell') \mid b_1 = 1\}$. Assume that the cops occupy $O^b(\ell)$. Then the 
robber is
blocked in the levels less or equal to $\ell$ (except that he can go to some 
$b_i(\ell')$, but he would be captured there immediately). Assume that there
are $|N(\ell)|+1$ free cops in that position. 

\begin{lemma}\label{lemma:cops_invariant}
For each $i\in\{0,1\}$, the cops have a strategy that allows them either to
capture the robber or to expel him from level~$\ell$ such that the
cops occupy precisely $O^b(\ell)\cup A(\ell) \cup \{b_i(\ell)\}$ for an 
$i\in\{0,1\}$. 
\end{lemma}
\begin{proof}
The strategy is as follows. One cop is placed on $c_{1-i}(\ell)$. This
creates two components of $S_\phi^\ell$: the one induced by $C_0(\ell)$ and the one
induced by $N(\ell)$, $A(\ell)$, $B(\ell)$, $C_i(\ell)$ and
$S_\phi^{\ell-3}$. If the robber is in $C_i(\ell)$, the remaining free cops
expel him from there and the robber is in the other component. Then
the cops occupy $N(\ell)$ and then the cop from $c_{1-i}(\ell)$
occupies $b_i(\ell)$. If the robber is in $C_i(\ell)$ and stays there,
he is captured there by the cops from $N(\ell)$, so assume that the
robber goes either to the component induced by $b_{1-i}(\ell)$
or to
the component induced by $A(\ell)$ and $S_\phi^{\ell-3}$. In any case the
cops leave $D(\ell)$ and occupy $A(\ell)$. If the robber remains
in $b_{1-i}(\ell)$, he is captured by the cop from $b_i(\ell)$, so
assume that he goes to $S_\phi^{\ell-3}$. We obtain the required
position. 
\end{proof}

\begin{lemma}\label{lemma:robber_invariant}
The robber has a strategy that permits him either to
win or to reach a position from position $P$ where the robber is in
$S_\phi^{\ell-3}$ and the cops occupy $O^b(\ell)$, $A(\ell)$ and at least 
one of $b_i(\ell)$. Furthermore, this robber strategy is winning if
there are only $|M(\ell)|$ free cops.
\end{lemma}
\begin{proof}
The robber stays in $N(\ell)$ until it is completely occupied by the
cops. In that position, one of $c_i(\ell)$ is not occupied by cops,
and the robber runs to a $C_i(\ell)$ and plays as
in the proof of Theorem~\ref{thm:super-poly}. Note that the cops from $A(\ell')$ 
and from $B(\ell')$
for all $\ell'>\ell$ cannot be removed.
\end{proof}


\begin{lemma}
  There is a winning strategy for $r+1$ cops on $S_\phi$ if and only if
  $\phi$ is true.
\end{lemma}
\begin{proof}
  Assume that~$r$ cops have a winning strategy~$\sigma$
  on~$S_\phi$. In $\MCGAME(\phi)$, the
  existential player simulates the cops and robber game on $S_\phi$ by
  translating the moves of the existential player into robber moves
  and translating cop moves (according to~$\sigma$) into his choices
  of the existentially quantified variables. Assume that we reached a
  position~$P$ in the cops and robber game and a position $P_i$ (for
  $i\ge 1$) in the $\MCGAME(\phi)$ sich that the following invariant (INV) holds.
\begin{itemize}
 \item the values $b_j = \beta(X_j)$ for the variables $X_j$ where 
$j\in\{1,\ldots,i-1\}$ are already chosen,

\item in the cops and robber game, the robber is in level $\ell = 
\ell(i)$ and

\item the cops occupy $O^b(\ell)$ for the tuple $b =
  (b_1,\ldots,b_{i-1})$ where $O^b(\ell)$ is defined as above. 
\end{itemize}
Then there are exactly $\ell+1$ free cops. If $Q_i = \forall$, the
universal player chooses a value $b_i = \beta(X_i)$ for $X_i$. Then
the existential player simulates the cops and robber game playing for
the cops according to~$\sigma$ from position~$P$ and for the robber as in
Lemma~\ref{lemma:robber_invariant} such that the robber is expelled
from level $\ell$ and $A(\ell)$ and $b_i(\ell)$ are occupied by cops. The number of
free cops suffices for that. It is straightforeward to check that the
above invariant holds for $i+1$ and for the position of the cops and
robber game where the robber is blocked in the next level, \ie in level~$\ell-3$.

If $Q_i = \exists$, the existential player simulates the cops and robber 
game from~$P$ until the robber is expelled from level~$\ell$ according to 
Lemma~\ref{lemma:cops_invariant}. Hereby, the cops play according
to~$\sigma$ and the robber plays arbitrarily, but such that he is not
captured in level~$\ell$. For example, the robber goes directly to
$S_\phi^{\ell -3}$.  Again, there are enough free cops for 
the simulation. Then exactly one of $b_0(\ell)$ and $b_1(\ell)\}$ is opccupied 
by a cop. If it is $b_0(\ell)$, the existential player sets $\beta(X_i) = 0$, 
otherwise $\beta(X_i) = 1$. Again, the invariant holds.

When all variables have their values, the universal player chooses a
clause~$C$ and the universal player simulates in the cops and robber
game the move of the free cop to vertex~$v$ in $F_\psi$ and the move
of the robber to~$K_C$. As the cops have played according to~$\sigma$
and~$\sigma$ is a winning strategy, there is a free cop. The cops completely 
occupy all $A(\ell)$ and for all
$\ell$ exactly one of $b_0(\ell)$ and $b_1(\ell)$. Every vertex in all
$A(\ell)$ is still reachable from the robber vertex, so the free cop
is in some $b_i(\ell)$. As the cop is free, there is no edge from any
$v_j^C$ to $b_i(\ell)$, \ie there is the edge from some $v_j^C$ to
$b_{1-i}(\ell))$. By construction of $S_\phi$, $X_j$ appears
in~$C$ and if $i=0$, then $X_j$ is negativ and if $i=1$, then
$X_j$ is positiv in~$C$. In the first case $b_i = 0$ and
$\beta(X_{v(\ell)}) = 0$, so~$C$ is satisfied and the existential
player wins by choosing $\neg X_j$. The second case is
symmetric.

For the other direction assume that the existential player has a winning 
strategy. We show that~$r$ cops have a winning strategy. The cops simulate 
the game $\MCGAME(\phi)$ while playing on $S_\phi$ by translating he moves of 
the 
robber to choices of the universal player and the choices of the existential 
player to their moves. Assume as before that (INV) holds for
some~$i\ge 1$.

There are two cases: level~$\ell$ is either existential or universal. In any 
case, there are $\ell + 1$ free cops and if the level is universal,~$\ell$ of 
them occupy $N(\ell)$. The robber escapes to some $C_i(\ell)$ for an $i\in 
\{0,1\}$ or goes to the component consisting of $A(\ell)$, $B(\ell)$ and 
$S_\phi^{\ell-3}$. If the robber is in $C_i(\ell)$ the last remaining cop is 
placed on $b_i(\ell)$ and the robber proceeds to $\{b_{1-i}(\ell)\}\cup 
A(\ell) \cup S_\phi^{\ell-3}$, otherwise the cop is placed on 
$b_i(\ell) = b_0(\ell)$ and the robber is in $\{b_1(\ell)\}\cup A(\ell) \cup 
S_\phi^{\ell-3}$. Now the cops from $D(\ell)$ occupy $A(\ell)$ and the robber 
goes to $S_\phi^{\ell-3}$ (if he goes to the free vertex of $B(\ell)$, he loses 
immediately). Finally, the cops simulate the choice of the universal player: 
$\beta(X_{v(\ell)}) = i$. It is easy to see that the invariant holds.

If the level is existential, the cops look up what value the strategy for the 
existential player in $\MCGAME(\phi)$ prescribes to choose for 
$X_{v(\ell)}$: $\beta(X_{v(\ell)}) = b_i \in \{0,1\}$. Then according to 
Lemma~\ref{lemma:cops_invariant} the cops can play such that the invariant 
holds again.

When the play arrives $F_\psi$, there is one free cop that is placed on~$v$ and 
the robber goes to some $K_C$ for a clause~$C$. As the existential player has a 
winning strategy, there is some literal $L_j$ in~$C$ that is satisfied 
by~$\beta$. Without loss of generality, $L_j = X_i$ and $\beta(X_i) = 1$. Then 
$b_1(\ell(i))$ is occupied by a cop, but there is no edge from~$v_i^C$ to 
$b_1(\ell(i))$. Recall that in $C$ every variable appears at most once, so 
there is no edge from~$C$ to $b_1(\ell(i))$ and the cop from $b_1(\ell(i))$ is 
free.
\end{proof}


==> taut.tex <==
\section{Reducing Tautology in CNF to \dagw}\label{sec:copnhard}

The construction of $G_n(s,t)$ shows how the robber can save the
history of the play in the current position. We extend it to reduce
the \taut problem to \DAGWprob (the problem, given a graph~$G$ and a
number~$k$, is $\DAGW(G)\le k$?).  \taut is the problem, given a
formula of propositional logic, to decide whether it is satisfied by
all variable interpretations. In general, \taut is \conp-hard, but in
our version the formula is given in CNF. This is a restriction, as
CNF-\taut is in \ptime, but we are going to extend our construction to
reduce QBF to \DAGWprob in Section~\ref{sec:pspace} where CNF is the
general case and which is more convenient for our purposes. We also restrict the
formulae by forbidding a variable to appear twice in a clause.

Let $\phi$ be a formula
with~$n$ variables and $m$ clauses. The graphs $H_\phi$ are based on
the graphs $G_m(s,t)$ such that
\begin{itemize}
\item the number of levels in $G_m(s,t)$ is one plus the number~$n$ of
  variables in~$\phi$,

\item $s(\ell) = \lfloor \log \ell \rfloor$ and $t(\ell)=2$ for all levels~$\ell$.
\end{itemize}

It will be convenient to define functions that relate variables and levels.
Let the variables of $\phi$ be enumerated as $X_1$, $X_2$, \ldots, $X_n$. Let 
$\ell\colon \{1,\ldots,n\} \to \{5,6,\ldots,m\}$ be an injection that maps the 
index of a variable to a level. Let $v$ be the function mapping a level to an 
index of a variable such that $v(\ell) = i$ if and only if $\ell(i) = \ell$.

We replace $G_4(s,t)$ (which is a single vertex) by the following
gadget~$F_\phi$. It has a vertex $v$ and for every clause $C=L_1 \lor
L_2 \lor \ldots L_{r(C)}$ an $r(C)$-clique $K_C$ with vertices $v_1^C$,
$v_2^C$, \ldots, $v^C_{r(C)}$. The edges go from $v$ to every vertex of
$K_C$ and back, \ie we have edges $(v,v_i^C)$ and $(v_i^C,v)$ for all
clauses $C$ and all $i\in\{1,\ldots,r(C)\}$. From outside of $F_\phi$, all 
vertices that had
outgoing edges to the vertex of $G_4(s,t)$ now have outgoing
edges to all vertices of $F_\phi$. So those edges build the set $A^s(\ell)
\times F_\phi \cup N(\ell)\times F_\phi$ for every level~$\ell$. Finally, the edges from $K_C$
leaving $F_\phi$ reflect the clause~$C$. For all levels $\ell$ 
if $X_j$ with $j=v(\ell)$ does not appear in~$C$, then there are edges
$(v_j^C,b_0(\ell))$ and $(v_j^C,b_1(\ell))$. If $X_j = L_i$
for some~$i\in\{1,\ldots,r(C)\}$, then there is an edge $(v_j^C,b_1(\ell))$. If
$\neg X_{v(\ell)} = L_i$, then there is an edge $(v_i^C,b_0(\ell))$. 

We claim that $n+1$ cops capture the robber in $H_\phi$ if and only if
$\phi$ is a tautology. Whether $\phi$ is a tautology or not, the cops
can play according to the strategy as in the proof of
Lemma~\ref{lemma:dagw} until the robber component is $F_\phi$. They
also have to follow that strategy up to irrelevant changes as was
shown in Theorem~\ref{thm:super-poly}. In that position exactly one
cop is free (the one that would capture the robber on $G_4(s,t)$ if we
played on $G_n(s,t)$) and the others occupy all $A^s(\ell)$ (in all
levels) and, in each level $\ell$, one of the two vertices $b_0(\ell)$
and $b_1(\ell)$. The free cop is placed on $v$ in $F_\phi$ (there is
no other legal move that does not lead to an immediate loss for the cops) and 
the robber chooses some $K_C$ for a clause
$C=L_1 \lor L_2 \lor \ldots L_r$. Let $X_{j_i}$ be the variable in the 
literal $L_i$. Now for all levels $\ell$ all cops 
from all $A^s(\ell)$
cannot be removed and reused as this would violate the monotonicity:
there are edges from all vertices of $K_C$ to all vertices of all
$A^s(\ell)$. The cops from every level $\ell$ such that $X_{v(\ell)}$ does
not appear in $C$ cannot be removed for the same reason. If one cop
from some $B^t(\ell)$ can be reused, the cops win as
follows. Let this cop be in level $\ell$ and assume without loss of
generality that $v(\ell) = j_1$. The cop is placed on $v_2^C$, then the cop 
from $B^t(\ell(j_2))$ is placed on $v_3^C$. Now the cop from
$B^t(\ell(j_3))$ is placed on $v_4^C$ and so on.

Then the following holds.
 
\begin{lemma}\label{lemma:use_one_cop}
The cops can win if and
only if they can reuse one of~$r$ cops from those~$r$ levels~$\ell$
in which $X_{v(\ell)}$ appears in~$C$.
\end{lemma}

Assume that $\phi$ is true under every valuation. Let $R\subseteq
\{1,\ldots,n\}$ be the set of indices~$v(\ell)$ of $X_{v(\ell)}$ appearing in
$C$. Let $\alpha\colon \{X_i \mid i\in R\} \to \{0,1\}^r$ be the
valuation of those $X_{v(\ell)}$ defined by the choices of the robber
during the play as follows. For all levels~$\ell$, if 
$X_{v(\ell)}$
appears in $C$ and the robber chose the component $C_i(\ell)$ in level
$\ell$ (for $i\in\{0,1\}$), then $\alpha(X_{v(\ell)}) = 1$ if $i=0$ and
$\alpha(X_{v(\ell)}) = 0$ if $i=1$. Let $\beta$ be a valuation of
$X_1,\ldots,X_n$ extending $\alpha$. As $\beta \models \phi$,
$\beta\models C$ and thus there is some $L_j$ in $C$ with $\beta
\models L_j$. Let $\ell$ be such that $X_{v(\ell)} = L_j$ or $\neg X_{v(\ell)} =
L_j$ (we have $v(\ell)\in R$). If $X_{v(\ell)} = L_j$, then $\beta(X_{v(\ell)}) 
=
\alpha(X_{v(\ell)}) = 1$ and thus the robber chose $C_0(\ell)$ in
level~$\ell$. Then a cop occupies $b_0(\ell)$, but there is no edge
from $K_C$ to $b_0(\ell)$ (there is an edge to $b_1(\ell)$), so the
cop from $b_1(\ell)$ can be reused and the cops win. If $\neg X_{v(\ell)} =
L_j$, the situation is symmetric.

If $\phi$ is not a tautology, let $\beta$ be a valuation with $\beta
\not\models \phi$. The robber winning strategy is to choose in level
$\ell$ the component $C_1(\ell)$ if $\beta(X_{v(\ell)}) = 0$ and the component
$C_0(\ell)$ otherwise. When the cops occupy $v$, the robber chooses the
component $F_C$ corresponding a clause $C = L_1 \lor \ldots \lor L_r$
with $\beta \not \models C$. Then $\beta \not \models L_j$ for all
$j\in\{1,\ldots,r\}$. Thus every cop in all $B^t(\ell)$ is still
reachable from the robber component and the cops lose. By 
Lemma~\ref{lemma:use_one_cop}, the cops win.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "bigDAGdecs"
%%% End: 

